Low-Complexity Multi-Antenna Coded Caching Using Location-Aware Placement Delivery Arrays

A location-aware multi-antenna coded caching scheme is proposed for applications with location-dependent data requests, such as wireless immersive experience, where users are immersed in a three-dimensional virtual world. The wireless connectivity conditions vary as the users move within the application area motivating the use of a non-uniform cache memory allocation process to avoid excessive delivery time for users located in wireless bottleneck areas. To this end, a location-aware placement and delivery array (LAPDA) is designed for cache-aided multiantenna data delivery with a fast converging, iterative linear beamforming process. The underlying weighted max-min transmit precoder design enables the proposed scheme to serve users in poor connectivity areas with smaller amounts of data while simultaneously delivering larger amounts to other users. Our new scheme is suitable for large networks due to its linear transceiver structure and it is not constrained by the number of users, cache size, or the number of antennas at the transmitter, unlike the existing schemes. Despite non-uniform cache placement, the proposed scheme still achieves a significant degree of coded caching gain that is additive to the multiplexing gain and greatly outperforms the conventional symmetric CC schemes in terms of both average and 95-percentile delivery time.

==> Delivery.tex <==
\section{Delivery}
\label{sec:delivery}
At the beginning of the delivery phase, every user $i \in \CK$ reveals its requested file $W_i \equiv W(s_i).$\footnote{Note that we have used $W(j)$ to represent the file required for reconstructing the FoV of the state $j$, and $W_i$ to denote the file requested by user~$i$. The same convention is used for all notations in the text.} Note that $W_i$ depends on the state $s_i$ where user $i$ is located. The server then builds and transmits several multiplexed codewords, such that after receiving the codewords, all users can reconstruct their requested files. From the system model, user $i$ requires a total amount of one normalized data unit to reconstruct $W_i$. However, a subset of this data, with size $m_i \equiv m(s_i)$ data units, is available in the cache of user $i$. In other words, user $i$ requires $K$ sub-files to reconstruct the original file and in total $t_i = t(s_i)$ sub-files are available at its cache. Since each user might be in a different state with distinct $t(j)$, the conventional delivery scheme of [MJ TWC] is no longer applicable, and a new delivery mechanism is required to achieve a proper multicasting gain.

Before continuing with the new algorithm, we first borrow some matrix representation from [MJ TWC]. Since users are in different states, we first calculate the minimum available caching gain among the users. Let us denote such a gain as $\hat{t}$, where $\hat{t} := \min_{i \in \CK} t_i$. Next, we define two Delivery Prime (DP) matrices $\BR_k$ and $\BC_k$, $k \in [K]$, with dimensions $(K-\hat{t}) \times (\hat{t}+L)$, based on which the delivery process is formed. $\BR_1$ and $\BC_1$ are built using Algorithms \ref{alg:R1_creation} and \ref{alg:C1_creation} (for all algorithms, $K, L, S, \hat{t}$ are assumed to be global variables known to the procedures); and for $k > 1$, we use circular increment to build $\BR_k$ and $\BC_k$ from $\BR_{k-1}$ and $\BC_{k-1}$, respectively. For an integer $a$, the intended circular increment operation in domain $K$ is defined as
\begin{equation}
    i_c (a,K) = (a \mod K) + 1 \; ,
\end{equation}
while for a matrix $\BA$ with positive integer elements, $i_c(\BA,K)$ results in a matrix in which each element is the circular increment (in domain $K$) of its respective element in $\BA$. Now for $k \in [2:K]$ we define
\begin{equation}
    \begin{aligned}
    \BR_k = i_c(\BR_{k-1},K) \; ; \;\; \BC_k = i_c(\BC_{k-1},K) \; .
    \end{aligned}
\end{equation}


\begin{algorithm}[t]
\caption{$\BR_1$ Generation Procedure}
\label{alg:R1_creation}
\begin{algorithmic}[1]
    \Procedure{Generate $\BR_1$}{}
        \ForAll{$j \in [1:\hat{t}]$}
            \ForAll{$i \in [1:K-2\hat{t}+j]$}
                \State $\BR_1 [i,j] \gets \hat{t}+i$
            \EndFor
            \ForAll{$i \in [K-2\hat{t}+j+1:K-\hat{t}]$}
                \State $\BR_1 [i,j] \gets i-(K-2\hat{t}+j-1)$
            \EndFor
        \EndFor
        \ForAll{$j \in [\hat{t}+1:\hat{t}+L]$, $i \in [1:K-\hat{t}]$}
            \State $\BR_1 [i,j] \gets 1$
        \EndFor
    \EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{$\BC_1$ Generation Procedure}
\label{alg:C1_creation}
\begin{algorithmic}[1]
    \Procedure{Generate $\BC_1$}{}
        \ForAll{$j \in [1:\hat{t}]$, $i \in [1:K-\hat{t}]$}
            \State $\BC_1 [i,j] \gets j$
        \EndFor
        \ForAll{$j \in [\hat{t}+1:\hat{t}+L]$, $i \in [1:K-\hat{t}]$}
            \If{$j+i-1 \le K$}
                \State $\BC_1 [i,j] \gets j+i-1$
            \Else
                \State $\BC_1 [i,j] \gets j+i-1-(K-\hat{t})$
            \EndIf
        \EndFor
    \EndProcedure
\end{algorithmic}
\end{algorithm}

The delivery process is done in $K$ phases, and during each phase $K-\hat{t}$ transmissions are performed. In this regard, the $j$'th row of $\BC_k$ determines the set of $\hat{t}+L$ users to be served during $j$'th transmission of $k$'th phase. To clarify the transmission content (file-chunks) of such a transmission, we use $j$'th row of $\BR_k$, but with some modifications as compared to [MJ TWC].

Selecting the subset of users for each transmission based on $\BC_k$, each user appears $(\hat{t}+L)\times(K-\hat{t})$ times during the $K$ phases [MJ TWC]. Since user $i \in [K]$ needs $K-t_i$ sub-files from the server to decode its intended data, each sub-file $W_{p}(s_i)$ is divided into $D_i = \alpha \frac{(\hat{t}+L)\times(K-\hat{t})}{K-t_i}$ file-chunks, where $\alpha \in \mathbb{N}$ is the smallest integer number such that $D_i \in \mathbb{N}, \forall i \in [K]$. The file-chunks of $W_{p}(s_i)$ are denoted by $\{W^{v}_{\CT_p}(s_i),  v \in [D_i]\}$, where $\CT_p(s_i)$ is defined as $\CT_p(s_i) := (p-1) \times i_c ([t_i],K)$, i.e., $p-1$ consecutive circular increment of the vector $\{1, \dots, t_i\}$. Note that $\CT_p(s_i)$ denotes the set of users, who have all the file-chunks $\{W^{v}_{\CT_p}(s_i), \forall v \in [D_i]\}$ available in their caches. Finally, $\sum_{i \in [K]}D_i(K-t_i)$ file-chunks are delivered to $K$ users following Algorithm \ref{alg:delivery_main}; with its auxiliary procedures presented in Algorithms \ref{alg:aux_init}, \ref{alg:aux_gen_r}, \ref{alg:sub_selection}, and \ref{alg:File_gen}. We have used $\{ \BC_k \} \equiv \{ \BC_1, ..., \BC_K \}$ and $\{ \BR_k \} \equiv \{ \BR_1, ..., \BR_K \}$; and \textsc{Modulate} function returns the modulated version of its input. The procedure is based on DP matrices. For each $k \in [K]$ we use $\BR_k$ and $\BC_k$ jointly, to create one transmission phase.

\begin{algorithm}[t]
\caption{Delivery Procedure}
\label{alg:delivery_main}
\begin{algorithmic}[1]
    \Procedure{Delivery}{$\{\BR_k \}, \{\BC_k \}$}
        \State \textsc{Initialize}
        \State $\hat{t} \gets \min_{i \in \CK} t_i$
        \ForAll{$i \in [K]$}
        \State $D_i \gets \alpha {(\hat{t}+L)\times(K-\hat{t})}/{(K-t_i)}$
            \State $W_{p}(s_i) \rightarrow \{W^{v}_{\CT_p}(s_i)  \; | \; \forall v \in [D_i] , \forall p \in [K]\}$
        \EndFor
        \ForAll{$k \in [K]$}
            \ForAll{$q \in [K-\hat{t}]$}
                \State $m \gets m+1$
                \State $\Bx(m) \gets 0$
                \ForAll{$j \in [\hat{t}+L]$}
                    \State $u \gets \BC_k[q,j]$
                    \State $r \gets \BR_k[q,j]$
                    \State $\CT \gets \textsc{Sub}\big(r, \hat{t}\big)$
                    \State $\CT_{d} \gets \{\CU , \ \CU \in \CT_{p}(s_u), \forall p \ | \ \CT \subseteq \CU, u \notin \CU\}$ \label{alg_lin:several file chunk}
                    \State $\hat{X} \gets $ \textsc{File-generator}$\big( \CT,\CT_{d}, \alpha, u \big)$
                    \State $\SfX \gets $ \textsc{Modulate}$\big( \hat{X} \big)$
                    \State $\CR \gets$ \textsc{Generate $\CR$}($\CT,\CT_d, u$)
                    \State $\Bx(m) \gets \Bx(m) + \Bv_{\CR} \SfX$
                    %\State $q \big( W(usr),prt \big) \gets q \big( W(usr),prt \big) + 1$
                \EndFor
                \State Transmit $\Bx(m)$
            \EndFor
        \EndFor
    \EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{Initialization Procedure}
\label{alg:aux_init}
\begin{algorithmic}[1]
    \Procedure{Initialize}{}
        \State $m \gets 0$
        \State ${\CT_c} \gets [\hat{t}]$
        \ForAll{$k \in [K]$}
        \State $\CT_k \gets [t_{s_k}]$
        \ForAll{$p \in [K]$}
            \State $v_{\CT_c}(k) \gets 1$
            \State $q_{\CT_k}(k) \gets 1$
            \State $\CT_k \gets i_c (\CT_k ,K)$
            \State ${\CT_c} \gets i_c ({\CT_c},K)$
            \EndFor
        \EndFor
    \EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{$\CR$ Generation Function}
\label{alg:aux_gen_r}
\begin{algorithmic}[1]
    \Function{Generate $\CR$}{$\CT,\CT_d, u$}
            \State $\CR \gets \{u \}$
                \If{$|\CT_d| = 1$}
                    \State $\CR \gets \CR \cup\CT_d$
                    \Else
                    \State $\CR \gets \CR \cup \CT$
                \EndIf
            \State \Return $\CR$
    \EndFunction
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{Subset selection Procedure}
\label{alg:sub_selection}
\begin{algorithmic}[1]
    \Function{\textsc{Sub}\big($r, \hat{t}$\big)}{}
        \State $\CT \gets [\hat{t}]$
        \State $x \gets 1$
        \While{$ x < r$}
            \State $\CT \gets i_c (\CT,K)$
            \State $x \gets x+1$
        \EndWhile
    \EndFunction
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
    \caption{File Generator Function}
    \label{alg:File_gen}
    \begin{algorithmic}[1]
        \Function{\textsc{File-generator}}{$\CT,\CT_{d}, \alpha, u$}
                \State $Y_{\CT, u} \gets 0$
                \ForAll{$c \in [\alpha]$}
                \State $x \gets v_{\CT}(u)$
                \State $\hat{\CT} \gets \CT_d(x)$
                \State $ind \gets q_{\hat{\CT}}(u)$
                \State $Y_{\CT, u} \gets$ \textsc{Concat} $ (Y_{\CT,u}, W_{\hat{\CT}}^{ind}(s_u))$
                \State $q_{\hat{\CT}}(u) \gets q_{\hat{\CT}}(u) +1$ \label{alg_step: file_index}
                \State $v_{\CT}(u) \gets i_c (v_{\CT}(u),|\CT_{d}|)$ \label{alg_step: chunk selection}
                \EndFor
            \State \Return $Y_{\CT, u}$
        \EndFunction
    \end{algorithmic}
\end{algorithm}


%The new delivery algorithm for the proposed setup is outlined in Algorithm~\ref{Alg:Delivery}. During the delivery phase, the server transmits a nested codeword $X_{\CU}$ for every subset of users $\CU$ with $|\CU|= \hat{t} +1$, where $\hat{t}$ is the \textit{common cache ratio} defined as $\hat{t} = \min_{i \in \CK} t_i$, and $t_i \equiv t(s_i)$. From the placement phase, we recall that the file $W_i$ intended for user $i \in \CU$ is split into sub-files $W_{\CV(s_i),i}$.
 
%Let us define $\CU_{-i} \equiv \CU \setminus \{i\}$ and consider a user $k \in \CU_{-i}$. All the sub-files $W_{\CV(s_i),i}$ for which $k \in \CV(s_i)$ are already available in the cache memory of user $k$. Thus, by transmitting (part of) every sub-file $W_{\CV(s_i),i}$ for which $\CU_{-i} \subseteq \CV(s_i)$ and $i \not\in \CV(s_i)$, a portion of $W_i$ is delivered to user $i$ without causing any interference at other users $k \in \CU_{-i}$.

\begin{exmp}
\label{exmp:interference-free-delivery}
Consider the network in Example~\ref{exmp:placement}, for which the cache placement is visualized in Figure~\ref{fig:cache pool}. Assume in a specific time slot, $s_1 = 1$, $s_2 =2$, $s_3 =3$, $s_4 = 4$. Denoting the set of requested sub-files for user $i$ with $\CM_i$ and assuming $A \equiv W(1)$, $B \equiv W(2)$, $C \equiv W(4)$, $D \equiv W(5)$, we have
\begin{equation}
    \begin{aligned}
    \CM_1 &= \{ A_{2}, A_{3}, A_{4} \}, \qquad
    \CM_2 = \{ B_{3}, B_{4}\}, \quad
    \CM_3 = \{ C_{4}\}, \quad
    \CM_4 = \{ D_{1}, D_{2}\}. 
    \end{aligned}
\end{equation}
Note that, the size of the sub-files of $A,B,C,D$ are $\frac{1}{4}$ data units; however, the number of required sub-files for each user (i.e., $|\CM_i| = K-t_i$) is different. The common cache ratio is $\hat{t} = 1$, and hence, during each transmission we deliver data to $\hat{t}+L = 3$ users. The total number of transmission phases is equal to $K = 4$, and DP matrices $\BR_k$ and $\BC_k$ are as follows
\begin{equation}
\label{eq:r1_exmp_1}
\begin{aligned}
    \BR_1 =
    \begin{bmatrix}
    2 & 1 & 1 \\
    3 & 1 & 1 \\
    4 & 1 & 1 
    \end{bmatrix}, 
    \; \BR_2 =
    \begin{bmatrix}
    3 & 2 & 2 \\
    4 & 2 & 2 \\
    1 & 2 & 2 
    \end{bmatrix}, 
    \; \BR_3 =
    \begin{bmatrix}
    4 & 3 & 3 \\
    1 & 3 & 3 \\
    2 & 3 & 3 
    \end{bmatrix}, 
    \; \BR_4 =
    \begin{bmatrix}
    1 & 4 & 4 \\
    2 & 4 & 4 \\
    3 & 4 & 4 
    \end{bmatrix}, \\
    \BC_1 =
    \begin{bmatrix}
    1 & 2 & 3 \\
    1 & 3 & 4 \\
    1 & 4 & 2
    \end{bmatrix}, 
    \;\BC_2 =
    \begin{bmatrix}
    2 & 3 & 4 \\
    2 & 4 & 1 \\
    2 & 1 & 3
    \end{bmatrix},
    \; \BC_3 =
    \begin{bmatrix}
    3 & 4 & 1 \\
    3 & 1 & 2 \\
    3 & 2 & 4
    \end{bmatrix},
    \; \BC_4 =
    \begin{bmatrix}
    4 & 1 & 2 \\
    4 & 2 & 3 \\
    4 & 3 & 1
    \end{bmatrix}.
\end{aligned}
\end{equation}
%, and we need $\binom{4}{2} = 6$ transmissions in total. 
Based on the delivery procedure detailed in Algorithm~\ref{alg:delivery_main}, the requested sub-files of user $i$ are first divided into $D_i = \alpha \frac{(\hat{t}+L)\times(K-\hat{t})}{K-t_i}$ file-chunks. As the result, the sub-files in $\CM_i$ will be divided as follows
\begin{equation} \label{ex: file-chunks}
    \begin{aligned}
    \CM_1 &= \{ A^{v_1}_{\{2\}}, A^{v_1}_{\{3\}}, A^{v_1}_{\{4\}} \}, \ {v_1} \in [6], \quad
    \CM_2 = \{ B^{v_2}_{\{3,4\}}, B^{v_2}_{\{4,1\}}\}, \ {v_2} \in [9], \\
    \CM_3 &= \{ C^{v_3}_{\{4,1,2\}}\}, \ {v_3} \in [18], \quad
    \CM_4 = \{ D^{v_4}_{\{1,2\}}, D^{v_4}_{\{2,3\}}\} \ {v_4} \in [9], 
    \end{aligned}
\end{equation}
where $D_1 = 6, D_2 = D_4 = 9, D_3 = 18$, and $\alpha$ is equal to $2$. From~\eqref{ex: file-chunks} it is clear that there exist $D_i(K-t_i) = \alpha(\hat{t}+L)(K-\hat{t}) = 18$ file-chunks to be transmitted to each user. Based on the delivery procedure, in each transmission, we target $\hat{t}+L = 3$ users, where for each user in the targeted group a data comprised of $\alpha$ file-chunks is transmitted. As the result, the size of the transmitted data intended for user $1,2,3$ and $4$ is equal to $\frac{1}{12}, \frac{1}{18}, \frac{1}{36}$ and $\frac{1}{18}$, respectively. Note that the size of the intended data towards each user is proportional to the approximated rate of its location, i.e., the users in locations with better channel conditions are served with larger data sizes compared to those in poor-conditioned locations.

%Let us consider the case $\CU = \{1,2\}$. The codeword $X_{12}$ is supposed to deliver a portion of the requested data to users $1$ and $2$ interference-free. This is done by including (parts of) $A_{2}$, $B_{13}$, $B_{14}$ in $X_{12}$. As can be seen from Figure~\ref{fig:cache pool}, user $1$ has $B_{13}$ and $B_{14}$ in its cache memory, and so it can remove them from its received data and decode (part of) $A_{2} \in \CT_1$ interference-free. Similarly, user $2$ can remove $A_{2}$ using its cache contents and decode (parts of) $B_{13},B_{14} \in \CT_2$ interference-free. The coding procedure is explained in more details in Example~\ref{exmp:coding-procedure}.
\end{exmp}

As illustrated in Example~\ref{exmp:interference-free-delivery}, due to the proposed location-dependent cache placement, the value of $t_i$ (and hence, the total number of required sub-files) might differ for various users. To tackle this issue, the sub-files intended for different users are divided into distinct number of file-chunks, such that the total number of file-chunks required by each user is the same. Moreover, based on step~\ref{alg_lin:several file chunk} in Algorithm~\ref{alg:delivery_main}, we may find several candidate file-chunks which can be transmitted to a user in a single transmission. We address this issue by introducing an auxiliary Algorithm~\ref{alg:File_gen} with its auxiliary function $\textsc{Chunk}$. Whenever there exist more than one suitable file-chunk (i.e., $|\CT_d| > 1$) for a user, we \textit{concatenate} $\alpha$ file-chunks from different subsets in $\CT_d$ following step~\ref{alg_step: chunk selection} (Algorithm~\ref{alg:File_gen}) to create the part of $X(m)$ intended for user $u$, represented by $Y_{\CT,u}$. The variable $q_{\hat{\CT}}(u)$ in step~\ref{alg_step: file_index} (Algorithm~\ref{alg:File_gen}), ensures none of the file-chunks of a sub-file is sent twice, and the function $\textsc{Concat}$ creates a bit-wise concatenation of the given file-chunks. The final codeword $\hat{X}$ is then modulated to create $\SfX$, then multiplied by its appropriate precoder $\Bv_{\CR}$ and multiplexed with the message of other intended users. As we discuss in section (XXX), the optimal precoder $\Bv_{\CR}$ is designed based on weighted-max-min rate optimization.

\begin{exmp}
\label{exmp:coding-procedure}
Following Example~\ref{exmp:interference-free-delivery}, let us review how the downlink message $\Bx(m)$ is built in each transmission. Following the DP matrix $\BC_1$, the first transmission targets user $1,2$ and $3$. Now, based on $\BR_1$, the intended file for user $1$ should contain file-chunks with index including $\{2\}$ and excluding $\{1\}$. Therefore, the only file-chunk candidates are $\{A^{v_1}_{\{2\}}, v_1 \in [6]\}$. Therefore the intended message for user $1$ is $Y_{\{2\}, 1} = \textsc{Concat} (A_{\{2\}}^{1}, A_{\{2\}}^{2})$. Similarly, we can write the intended message for user $2$ and $3$ as $Y_{\{1\}, 2} = \textsc{Concat} (B_{\{4,1\}}^{1}, B_{\{4,1\}}^{2})$ and $Y_{\{1\}, 3} = \textsc{Concat} (C_{\{4,1,2\}}^{1}, C_{\{4,1,2\}}^{2})$. Therefore, the first transmitted message is as follows
\begin{equation} \label{eq:first_transmission}
    \Bx(1) = \Bv_{\{1,2\}}[A_{\{2\}}^{1} \ A_{\{2\}}^{2}] +  \Bv_{\{1,2,4\}} [B_{\{4,1\}}^{1} \ B_{\{4,1\}}^{2}] +  \Bv_{\{1,2,3,4\}}[C_{\{4,1,2\}}^{1} \ C_{\{4,1,2\}}^{2}] \; ,
\end{equation}
where $[A \ B]$ denotes the modulated version of $\textsc{Concat} (A, B)$. According to~\eqref{eq:first_transmission}, the received signal at user $1$ is as follows
\begin{equation}
\label{eq:first_reception}
        y_1(1) = [A_{\{2\}}^{1} \ A_{\{2\}}^{2}] \Bh_1^T \Bv_{\{1,2,4\}} +  \underline{[B_{\{4,1\}}^{1} \ B_{\{4,1\}}^{2}] \Bh_1^T \Bv_{\{1,2\}}} + \underline{[C_{\{4,1,2\}}^{1} \ C_{\{4,1,2\}}^{2}] \Bh_1^T \Bv_{\{1,2,3,4\}}} + w_1(1) \; ,
\end{equation}
where $w_1(1)$ denotes the receiver noise. Since the underlined content are available in the cache of user $1$, by estimating $\Bh_1^{T} \Bv_{\CR}$, these content can be removed from the received signal and $[A_{\{2\}}^{1} \ A_{\{2\}}^{2}]$ can be decoded interference free [MJ TWC]. Now, for ease of exposition, assume  zero-forcing beamformers \footnote{The general beamformer design is discussed in details in section (XXX).} $\Bv_{\CR}$ are used to build $\Bx(1)$, where $\CR \subseteq \BC_1(1,:)$;
and $\Bv_{\CR}$ is built such that $\|\Bv_{\CR}\| = 1$ and
\begin{equation}
\label{eq:zeroforce_definition}
    \begin{aligned}
    \Bh_k^T \Bv_{\CR} &\neq 0 \qquad k \in \CR \; , \\
    \Bh_k^T \Bv_{\CR} &= 0 \qquad \BC_1(1,:) \backslash \CR \; .
    \end{aligned}
\end{equation}
As the result, the received signal at user $2$ and $3$ is as follows
\begin{equation}
\begin{aligned}
        y_2(1) &=  {[B_{\{4,1\}}^{1} \ B_{\{4,1\}}^{2}] \Bh_2^T \Bv_{\{1,2,4\}}} + \underline{[A_{\{2\}}^{1} \ A_{\{2\}}^{2}] \Bh_2^T \Bv_{\{1,2\}}} + \underline{[C_{\{4,1,2\}}^{1} \ C_{\{4,1,2\}}^{2}] \Bh_2^T \Bv_{\{1,2,3,4\}}} + w_2(1) \; , \\
        y_3(1) &= [C_{\{4,1,2\}}^{1} \ C_{\{4,1,2\}}^{2}] \Bh_3^T \Bv_{\{1,3\}} + w_3(1) \; .
\end{aligned}
\end{equation}
Following similar argument as for user $1$, users $2$, and $3$ can decode their intended data interference free. Similarly, the rest of the transmitted message in first phase is as follows
\begin{equation} \label{eq:second&third transmissions}
\begin{aligned}
    \Bx(2) &= \Bv_{\{1,3\}}[A_{\{3\}}^{1} \ A_{\{3\}}^{2}] +  \Bv_{\{1,2,3,4\}} [C_{\{4,1,2\}}^{3} \ C_{\{4,1,2\}}^{4}] +  \Bv_{\{1,2,4\}}[D_{\{1,2\}}^{1} \ D_{\{1,2\}}^{2}] \; , \\
    \Bx(3) &= \Bv_{\{1,4\}}[A_{\{4\}}^{1} \ A_{\{4\}}^{2}] +  \Bv_{\{1,2,4\}} [D_{\{1,2\}}^{3} \ D_{\{1,2\}}^{4}] +  \Bv_{\{1,2,4\}}[B_{\{4,1\}}^{3} \ B_{\{4,1\}}^{4}] \; ,
\end{aligned}
\end{equation}
Now, for the forth transmission, which corresponds to the first row of $\BC_2$, we target users $2,3$ and $4$. Based on $\BR_2$, the intended file for user $2$ should contain file-chunks with index including $\{3\}$ and excluding $\{2\}$. Therefore, the only file-chunk candidates are $\{B^{v_2}_{\{3,4\}}, v_2 \in [9]\}$. Similarly, the only candidate file-chunks for user $3$ are $\{C^{v_3}_{\{4,1,2\}}, v_2 \in [18]\}$. However, the intended file for user $4$ should contain file-chunks with index including $\{2\}$ and excluding $\{4\}$, which leaves us with two sets of file-chunks $\{D^{v_4}_{\{1,2\}}, v_4 \in [9]\}$ and $ \{D^{v_4}_{\{2,3\}}, v_4 \in [9]\}$ (i.e., $|\CT_d| = 2$). Therefore the intended message for user $4$ is $Y_{\{2\}, 4} = \textsc{Concat} (D^{5}_{\{1,2\}}, D^{1}_{\{2,3\}})$. As the result, the remaining transmitted messages can be expressed as follows
\begin{equation}
    \begin{aligned}
    \Bx(4) &= \Bv_{\{2,3,4\}}[B_{\{3,4\}}^{1} \ B_{\{3,4\}}^{2}] +  \Bv_{\{1,2,3,4\}} [C_{\{4,1,2\}}^{5} \ C_{\{4,1,2\}}^{6}] +  \Bv_{\{2,4\}}[D_{\{1,2\}}^{5} \ D_{\{2,3\}}^{1}] \; , \\
    \Bx(5) &= \Bv_{\{2,4\}}[B_{\{4,1\}}^{5} \ B_{\{3,4\}}^{3}] +  \Bv_{\{2,4\}}[D_{\{1,2\}}^{6} \ D_{\{2,3\}}^{2}] +  \Bv_{\{1,2\}}[A_{\{2\}}^{3} \ A_{\{2\}}^{4}] \; , \\
    \Bx(6) &= \Bv_{\{1,2,4\}}[B_{\{4,1\}}^{6} \ B_{\{4,1\}}^{7}] +  \Bv_{\{1,2\}}[A_{\{2\}}^{5} \ A_{\{2\}}^{6}] +  \Bv_{\{1,2,3,4\}} [C_{\{4,1,2\}}^{7} \ C_{\{4,1,2\}}^{8}] \; , \\
    \Bx(7) &= \Bv_{\{1,2,3,4\}}[C_{\{4,1,2\}}^{9} \ C_{\{4,1,2\}}^{10}]  +  \Bv_{\{2,3,4\}} [D_{\{2,3\}}^{3} \ D_{\{2,3\}}^{4}] +  \Bv_{\{1,3\}}[A_{\{3\}}^{3} \ A_{\{3\}}^{4}] \; , \\
    \Bx(8) &= \Bv_{\{1,2,3,4\}}[C_{\{4,1,2\}}^{11} \ C_{\{4,1,2\}}^{12}] +  \Bv_{\{1,3\}}[A_{\{3\}}^{5} \ A_{\{3\}}^{6}] +  \Bv_{\{2,3,4\}}[B_{\{3,4\}}^{4} \ B_{\{3,4\}}^{5}] \; , \\
    \Bx(9) &= \Bv_{\{1,2,3,4\}} [C_{\{4,1,2\}}^{13} \ C_{\{4,1,2\}}^{14}] +  \Bv_{\{2,3,4\}}[B_{\{3,4\}}^{6} \ B_{\{3,4\}}^{7}] +  \Bv_{\{2,3,4\}} [D_{\{2,3\}}^{5} \ D_{\{2,3\}}^{6}] \; , \\
    \Bx(10) &= \Bv_{\{1,2,4\}} [D_{\{1,2\}}^{7} \ D_{\{1,2\}}^{8}] +  \Bv_{\{1,4\}}[A_{\{4\}}^{3} \ A_{\{4\}}^{4}] +  \Bv_{\{2,4\}}[B_{\{4,1\}}^{8} \ B_{\{3,4\}}^{8}] \; , \\
    \Bx(11) &= \Bv_{\{2,4\}}[D_{\{1,2\}}^{9} \ D_{\{2,3\}}^{7}] +  \Bv_{\{2,4\}}[B_{\{4,1\}}^{9} \ B_{\{3,4\}}^{9}] +  \Bv_{\{1,2,3,4\}}[C_{\{4,1,2\}}^{15} \ C_{\{4,1,2\}}^{16}] \; , \\
    \Bx(12) &= \Bv_{\{2,3,4\}} [D_{\{2,3\}}^{8} \ D_{\{2,3\}}^{9}] +  \Bv_{\{1,2,3,4\}}[C_{\{4,1,2\}}^{17} \ C_{\{4,1,2\}}^{18}] +  \Bv_{\{1,4\}}[A_{\{4\}}^{5} \ A_{\{4\}}^{6}] \; . \\
    \end{aligned}
\end{equation}
Note that all these transmissions can be decoded interference free following the same argument as in~\eqref{eq:first_transmission} and~\eqref{eq:second&third transmissions}.
\end{exmp}

\begin{thm}
Using the proposed cache placement and content delivery algorithms, every sub-file $\{W_{p}(s_i) , \; \forall p \in {K}\}$ needs to be divided to $D_i = \alpha \frac{(\hat{t}+L)\times(K-\hat{t})}{K-t_i}$ file-chunks, for the algorithm to work properly.
\end{thm}
\begin{proof}
A user $i \in \CK$ needs a total amount of $K$ sub-files to reconstruct its requested file $W_i$. If the user is in state $s_i$, $t_i$ number of sub-files are available in its cache memory, and hence it needs to receive $K-t_i$ sub-files from the server. As detailed in the delivery algorithm, user $i$ will be targeted $(\hat{t}+L)\times(K-\hat{t})$ times during the $K$ transmission phases [MJ TWC]. Each time user $i$ is targeted, a data comprised of file-chunks with superscript $\CT$ is delivered to him/her. Since there exist $K-\hat{t}$ distinct superscript, the $K-t_i$ sub-files must be divided among these transmissions. On the other hand, in some of these transmissions with particulate superscript $\CT_i(x)$ there may exist several file-chunks which can be delivered to user $i$, see example~\ref{exmp:coding-procedure}. Lets assume $\alpha_i(x)$ different sub-files can be delivered through superscript $\CT_i(x)$. As the result, we divide each sub-file into $D_i$ file-chunks, and we deliver $\frac{X(i)}{\alpha_i(x)}$ file-chunks from $\alpha_i(x)$ different candidates through superscript $\CT_x(i)$. Therefore, $\sum_{x = 1}^{K-\hat{t}}$ 
\end{proof}

==> Delivery_old.tex <==
\section{Content Delivery}
\label{sec:delivery}
During the delivery phase, users frequently change their locations over time.
In each time instance, users reveal their location-dependent file requests to the server.\footnote{Using dynamic coded caching techniques~\cite{salehi2021lowsubpacketization,abolpour2022coded}, this system model can be easily modified to the case only a subset of users reveal their requests in every time instant.} Without loss of generality, we consider a specific time slot, where every user $k$ in STU $s_k$ requests the file $W_{d_k} \equiv W(s_k)$ from the server to reconstruct its STU-specific FoV. Accordingly, the server builds and transmits several precoded messages to enable users to reconstruct their desired FoVs. To reconstruct $W(s_k)$, user $k$ requires one normalized data unit, from which a portion of size $m_k \equiv m(s_k)$ units is available in its cache and the remaining part should be delivered by the server. Note that the conventional PDA-based delivery schemes are suited for scenarios where all users cache the same amount of data (e.g.,~\cite{MLPDA_ISIT2022,lampiris2018adding,salehi2020lowcomplexity}). Thus, they do \textit{not} apply to the case where users have cached different amounts of their requested files. 

To address the challenge imposed by unequal cached data allocation, we first assume all users have the same amount of cached data equal to $\hat{m} = \min_{k \in \CK} m_k$ (note that in the placement phase, where the actual user locations are not yet known, the minimum allocated memory is calculated over all the STUs, i.e., $\bar{m} =  \min_{s \in \CS} m(s)$). Accordingly, we initially generate multiple primary transmission vectors. These vectors will be subsequently adjusted to account for the varying allocated memory requirements for the requested files.
%
%create a virtual network where all users have an equivalent amount of cached data. % and generate virtual transmission vectors. 
%For each virtual transmission vector, we construct an actual transmission vector using appropriate transformation matrices. In this regard, we first consider a virtual network in which all users have the same amount of cached data equal to $\hat{m} = \min_{k \in \CK} m_k$ (note that in the placement phase, where the actual user locations are not yet known, the minimum allocated memory is calculated over all the STUs, i.e., $\bar{m} =  \min_{s \in \CS} m(s)$). 
%
Using the \textit{min} operation may have limitations in certain scenarios when there are few users with relatively smaller $m(s_k)$ compared to the rest. This is especially evident when there are few users in close proximity to the transmitter. To address the situation, the concept of phantom users has been proposed in~\cite{mahmoodi2022asymmetric_arxiv_TWC2023}, which involves serving users with low available memory separately.

Assuming every user has the same cached data, every conventional PDA-based delivery scheme (e.g.,~\cite{MLPDA_ISIT2022,lampiris2018adding,salehi2020lowcomplexity}) can be readily used for data delivery. In this regard, we use the MLPDA $\hat{\BQ}$ corresponding to the location of the user with the least available memory, i.e., $\hat{\BQ} \equiv \BQ_{s_{k^{*}}}$, $k^{*} := \arg\min_{k \in \CK} m(s_k)$, to build primary transmission vectors. For clarity, we designate $\Check{\Bx}_{\CU}$ to represent primary transmission vectors, which will be later modified to form actual transmission vectors $\Bx_{\CU}$ (the same convention is also used for the other parameters and variables). 
%However, during the delivery phase, the users' actual locations are known, and we use $\hat{m} =  \min_{k \in \CK} m_k$ to take the minimum over all the users' locations). Now, every conventional PDA-based delivery scheme (e.g.,~\cite{MLPDA_ISIT2022,lampiris2018adding,salehi2020lowcomplexity}) can be readily applied to the virtual network. In this regard, we use the MLPDA $\hat{\BQ}$ corresponding to the location of the user with the least available memory, i.e., $\hat{\BQ} \equiv \BQ_{s_{k^{*}}}$, $k^{*} := \arg\min_{k \in \CK} m(s_k)$, to build transmission vectors for this virtual network. For clarity, we use $\Check{\Bx}_{\CU}$ to denote the virtual counterpart of the actual transmitted signal $\Bx_{\CU}$ (the same convention is also used for the other parameters and variables).
Specifically, users are served in $\hat{N} = N_{s_{k^{*}}}$ consecutive transmissions, where the primary transmission vector at time instant $n \in [\hat{N}]$ is
\begin{equation}\label{eq: multiplexed signal}
    \Check{\Bx}(n) \equiv \Check{\Bx}_{{\CU}(n)} = \sum_{k \in \CU(n)}\Bv_{k}(n)W_{\Check{f}_k^n}(s_k) \; , 
\end{equation}
where 
\begin{equation} \label{eq:Target_user_set}
{\CU}(n):=\{k \ | \ \exists \Check{f}_k^n \in [F], \ \hat{\BQ}(\Check{f}_k^n,k) = n\}
\end{equation}
is the set of users served in the $n$'th transmission, $\Check{f}_k^n$ is the virtual index of subfile transmitted to user $k \in \CU(n)$, and $\Bv_{k}(n)$ is the optimized beamforming vector dedicated to user $k$. Specifically, $\Bv_{k}(n)$ is designed to suppress $W_{\Check{f}_k^n}(s_k)$ at every user in $\CI_k(n)$, where 
\begin{equation}\label{eq:Interference_inc_set}
    \CI_k(n) = \{j \, | \, j \in \CU(n)\setminus k, \, \hat{\BQ}(\Check{f}_k^n,j) \neq \ast\}
\end{equation} 
is the interference indicator set. In other words, $\CI_k(n)$ collects all users $j \in \CU(n)\setminus k$ that do not have $W_{\Check{f}_k^n}(s_k)$ available in their cache memories. After the transmission of $\Bx_{\CU(n)}$, the corresponding received signal at user $k \in \CU(n)$ is given in~\eqref{eq:recieved_signal_sysmodel}. It is worth noting that the transmission vectors $\Check{\Bx}(n)$ are built for the virtual network, hence, in the real network, the subfile $\Check{f}_k^n$ may not exist or may already be available in the user's cache. This is clarified by the following example. 
\begin{exmp}
\label{exmp:virt_network}
Consider the network in Example~\ref{exmp:placement}, for which the cache placement is illustrated in~\eqref{eq:LAPDA_example}. %Figure~\ref{fig:cache pool}. 
Assume in a specific time instant $n$ the following user-to-STU association, $s_1 = 1$, $s_2 =2$, $s_3 =3$, $s_4 = 4$. Denoting the set of requested sub-files for user $k$ with $\CM_k$ and assuming $A \equiv W(1)$, $B \equiv W(2)$, $C \equiv W(4)$, $D \equiv W(5)$, we have
\begin{equation}
    \begin{aligned}
    \CM_1 &= \{ A_{4}, A_{5}, A_{6}, A_{7}, A_{8}, A_{9}, A_{10}, A_{11}, A_{12} \}, \\ 
    \CM_2 &= \{ B_{3}, B_{4}\}, \quad
    \CM_3 = \{ C_{4}\}, \quad
    \CM_4 = \{ D_{1}, D_{2}\}. 
    \end{aligned}
\end{equation}
Note that the subfiles of $A, B, C, D$ are $1/12,1/4,1/4,1/4$ data units in size, respectively. Here, the minimum available cache belongs to user $1$; hence, $\hat{\BQ} \equiv \BQ_1$, and we serve all users in $\hat{N} = N(1) = 12$ time slots. According to $\hat{\BQ}$ and~\eqref{eq: multiplexed signal}, the first four virtual transmissions are built as follows
\begin{equation*}
    \begin{aligned}
        \Check{\Bx}(1) &= \Bv_{1}(1) A_4+\Bv_{2}(1) B_1+\Bv_3(1) C_1, \ \quad \Check{\Bx}(2) = \Bv_1(2) A_7+\Bv_3(2) C_2+\BV_4(2) D_1,\\
        \Check{\Bx}(3) &= \Bv_1(3) A_{10}+\Bv_2(3) B_2+\Bv_4(3) D_2, \quad \Check{\Bx}(4) = \Bv_2(4) B_7 +\Bv_3(4) C_4+\Bv_4(4) D_4. 
    \end{aligned}
\end{equation*}
As an example, ${\CU}(1)= \{1,2,3\}$ can be obtained easily based on~\eqref{eq:LAPDA_example} and~\eqref{eq:Target_user_set}, indicating that the first transmission is directed toward users  $1$, $2$, and $3$. Similarly, the beamformers $\Bv_{1}(1)$, $\Bv_{2}(1)$ and $\Bv_{3}(1)$ should be designed to suppress interference towards users $\CI_{1}(1) = \{3\}$, $\CI_{2}(1) = \{3\}$, and $\CI_{3}(1) = \{2\}$, respectively, as indicated by~\eqref{eq:LAPDA_example} and~\eqref{eq:Interference_inc_set}. Other transmission vectors and sets can be easily obtained in a similar manner. %The remaining eight transmissions $\Check{\Bx}(5)-\Check{\Bx}(12)$ are formed in a similar manner. 
Considering $\Check{\Bx}(1)-\Check{\Bx}(4)$, we can see that subfiles $\{B_1, B_2, C_1, C_2, D_4\}$ are already available in the users' caches, and subfile $B_7$ does not exist.
\end{exmp}
Example~\eqref{exmp:virt_network} demonstrates that $\hat{\BQ}$ cannot be directly used to provide missing data to users in the real network. To address this, an elevation mechanism is employed to convert the virtual subfile indexes into the appropriate actual missing subfile indexes. Specifically, the DL message $\Bx(n)$ in the $n$-th transmission is built as
\begin{equation}\label{eq:original data vector}
    \Bx(n) = \sum_{k \in \CU(n)}\Bv_{k}\underset{{m \in [\alpha]}}{\prod}\left(W^q_{\BP_k(n,m)}(s_k)\right) \; 
\end{equation}
where $\prod$ denotes the bit-wise concatenation operation, and $q$ is the file-fragment index which is initialized to one and increased every time a file-fragment appears in a transmission vector. Also, $\alpha$ and $\BP_k$ are the \emph{stretch factor} and the \emph{user-specific file-fragment index matrix} for the elevation process, respectively. 
%
The process to create $\BP_k = [\BP_k(n,m)], n \in [\hat{N}], m \in [\alpha]$ will be explained shortly after. The need for the $\alpha$ parameter stems from the fact that each user $k$ receives $\hat{F}-\hat{Z}$ subfiles in virtual transmissions $\Check{\Bx}(1)-\Check{\Bx}(\hat{N})$, where $\hat{Z} \equiv Z_{s_{k^*}}$ and $\hat{F} \equiv F_{s_{k^*}}$. But, as the actual number of missing subfiles for user $k$ to decode its FoV is $F_{s_k}-Z_{s_k}$, we need to divide each subfile into $\hat{D}_k = \frac{\hat{F}-\hat{Z}}{F_{s_k}-Z_{s_k}}$ file-fragments to uniformly map the actual missing subfiles $f_{s_k} \in [F_{s_k}]$ into virtual subfile indexes $\Check{f}_k^n \in [\hat{F}]$ in the virtual network. Now, because $\hat{D}_k$ is not necessarily an integer for all $k \in \CK$, we use $\alpha$ to guarantee that $D_k = \alpha \hat{D}_k$ is an integer for all $k$.

After finding $\alpha$, each subfile $W_{f_{s}}(s_k)$ is divided into $D_k$ file-fragments, i.e., 
\begin{equation} \label{File-fragment division}
    W_{f_{s}}(s_k) \rightarrow \{W^{\phi}_{f_{s}}(s_k) \ | \ \phi \in [D_k]\}.
\end{equation}
Note that, with this adjustment, the total number of delivered file-fragments to user $k$ is equal to $D_T = (F_{s_k}-Z_{s_k})D_k = \alpha(\hat{F}-\hat{Z})$, which is STU independent. The elevation process in~\eqref{eq:original data vector} implies that every virtual subfile $ W_{\Check{f}_k^n}(s_k)$ in $\Check{\Bx}(n)$ is replaced by the bit-wise concatenation of $\alpha$ file-fragments 
$W^q_{\BP_k(n,m)}(s_k)$ in $\Bx(n)$, i.e.,
\begin{equation}\label{virtual_index_replacement}
    W_{\Check{f}_k^n}(s_k) \rightarrow \underset{{m \in [\alpha]}}{\prod}\left(W^q_{\BP_k(n,m)}(s_k)\right) ,
\end{equation} 
where, $\BP_k(n,m) \in [F_{s_k}]$.
%
The file-fragment indexes $\BP_k(n,m)$ are constructed such that 1) all the missing subfiles are delivered to all the users and 2) the cache-aided interference cancellation is correctly made. To build $\BP_k$, we first form $K$ user-specific File-Mapping (FM) matrices $\BG_k, \forall k \in [K]$, with size $\hat{F} \times F_k$, to map the actual missing subfiles to their virtual counterparts. The matrix elements are denoted by $g_{i,j,k}$, where $g_{i,j,k}$ belongs to the $i$'th row and $j$'th column of the matrix $\BG_k$. The element $g_{i,j,k}$, indicates how many file-fragments of $W_{j}(s_k), j \in [F_{s_k}]$ should be substituted for virtual subfile $W_{i}(s_k), i \in [\hat{F}]$ (the formal definition is provided shortly in Definition~\ref{FM_matrix_definition}). 

Insert the definition here. ... In order to solve this a system of equations need to be solved... Appendix A.

Finally, after $\{\BG_k\}$ are formed, $\{\BP_k\}$ are built using the process outlined in Algorithm~\ref{alg:File_ind_gen}. In a nutshell, in each round $n \in [\hat{N}]$ and $m \in [\alpha]$, a file-fragment of $W_\omega(s_{k}), k \in \CU(n)$ is assigned to $\BP_k(n,m)$ if $g_{\Check{f}_k^n, \omega, k}$ is positive and  $g_{\Check{f}_k^n, \omega, k}$ is subtracted by $1$ for the following rounds.

\begin{algorithm}[t]
    \caption{File-Fragment Index Matrix}
    \label{alg:File_ind_gen}
    \begin{algorithmic}[1]
        \Function{\textsc{Index-generator}}{$\{\BG_k\}, \hat{\BQ}$}
        \ForAll{$k \in [K]$}
            \State $\BP_k \gets \mathbf{0}$
        \EndFor
         \ForAll{$n \in [\hat{N}]$}
                    \ForAll{$k \in \CU(n)$}
                        \State $\chi \gets \Check{f}_k^n$
                        \ForAll{$m \in [\alpha]$}
                            \ForAll{$\omega \in [F_{s_k}]$}
                                \If{$g_{\chi,\omega,k} > 0$}
                                    \State $\BP_{k}(n,m) \gets \omega$
                                    \State $g_{\chi,\omega,k} \gets g_{\chi,\omega,k}-1$
                                    \State Break;
                                \EndIf
                            \EndFor
                        \EndFor
                    \EndFor
          \EndFor
            \State \Return $\{\BP_k\}$
        \EndFunction
    \end{algorithmic}
\end{algorithm}

Formal FM matrix formation is illustrated in Appendix~\ref{sec: Appendix A} by solving systems of equations. In general, an FM matrix $\BG_k$ is defined as follows. 
\begin{definition} \label{FM_matrix_definition}
A user-specific FM matrix $\BG_k = \left[g_{i,j,k}\right], \ \forall i \in [\hat{F}], j \in [F_{s_k}], k \in [K]$ is a $\hat{F} \times F_{s_k}$ matrix whose elements are comprised of non-negative integers, and satisfy the followings:
\begin{enumerate}
  \item[C1.] 
  Denoting the set of virtual subfiles delivered to user $k$ as a dedicated index set (DIS) $\Check{\CN}_{k}$ (i.e., $|\Check{\CN}_{k}| = \hat{F}-\hat{Z}$), every row of $\BG_k$ not included in $\Check{\CN}_{k}$ should be zero, i.e.,
  %The different virtual subfiles assigned to user $k$ constitute a dedicated index set (DIS) $\Check{\CN}_{k}$, where $|\Check{\CN}_{k}| = \hat{F}-\hat{Z}$. The elements in rows not included in DIS are all set to zero, i.e., 
  \begin{equation*}
      g_{i,j,k} = 0, \quad \forall k \in [K],  \ \forall i \in [\hat{F}] \setminus \Check{\CN}_{k},  \ \forall j \in [F_{s_k}].
  \end{equation*}
  \item[C2.] 
  %Following the cache placement proposed in section~\ref{sec:cache_placement}, every file $W(s_k)$ is divided into $F_{s_k}$ subfiles, from which $Z_{s_k}$ ones are available in the cache memory of user $k$ in state $s_k$, and $F_{s_k}-Z_{s_k}$ missing subfiles should be delivered by the BS.
  Denoting the set of missing subpackets of user $k$ in STU $s_k$ as a requested index set (RIS) $\CN_k$ (i.e., $|\CN_k| = F_{s_k}-Z_{s_k}$), the columns of $\BG_k$ not included in $\CN_k$ should be zero, i.e., 
  \begin{equation*}
      g_{i,j,k} = 0, \quad \forall k \in [K], \ \forall j \in [F_{s_k}] \setminus \CN_k, \ \forall i \in [\hat{F}].
  \end{equation*}
  \item[C3.] Based on Definition~\ref{MLPDA_definition_new}, each virtual subfile $i \in \Check{\CN}_{k}$ appears once during $\hat{N}$ transmissions. Thus, from $D_T$ missing file-fragments of user $k$, $\frac{D_T}{\hat{F}-\hat{Z}} = \alpha$ file-fragments should be substituted for each virtual subfile in $\Check{\CN}_{k}$, i.e., 
  \begin{equation*}
      \sum_{j \in \CN_k}g_{i,j,k} = \alpha, \quad \forall k \in [K], \ \forall i \in \Check{\CN}_{k}.
  \end{equation*}
  %which constitute a requested index set (RIS) $\CN_k$, where $|\CN_k| = F_{s_k}-Z_{s_k}$. Thus, the $g_{i,j,k}$ elements in the columns of $\BG_k$ not included in RIS are all set to zero, i.e., 
  \item[C4.] Based on~\eqref{File-fragment division}, each subfile $f_{s_k} \in \CN_k$ is divided into $D_k$ file-fragments. Thus, to make sure that all $D_k$ missing file-fragments are delivered to each user, the sum of the elements in every column of $\BG_k$ included in RIS must be equal to $D_k$, i.e., 
  \begin{equation*}
      \sum_{i \in \Check{\CN}_k}g_{i,j,k} = D_k, \quad \forall k, \ \forall j \in \CN_k.
  \end{equation*}
\end{enumerate}
\end{definition}
Lastly, the following example illustrated the elevation process, which is summarized in Algorithm~\ref{Alg:Delivery_main}.
\begin{algorithm}[ht]
\small
    \caption{Location-dependent CC-Aided Delivery}
	\begin{algorithmic}[1]
		\Procedure{DELIVERY}{$\{\BQ_k\}$}
		
		\State $k^{*} = \arg\min_{k \in \CK} m_k$
            \State $\hat{\BQ} \gets \BQ_{k^{*}}$
            \ForAll{$k \in [K]$}
            \State Form $\BG_k$ based on $\hat{\BQ}$
            \State Compute $\BP_k$ based on $\BG_k$ using Algorithm~\ref{alg:File_ind_gen}
            \EndFor
		\ForAll{$n \in [\hat{N}]$} %\label{alg:delivery_K_subsets}
		\If{$|\CU(n) \setminus \CK_p| \geq L$} \label{alg:phantom_DoF_check}
		\State $\Bx(n) \gets 0$
		        \ForAll{$k \in \CU(n) \setminus \CK_p$}
                    \State $x_{k} \gets 0$
		            \ForAll{$m \in [\alpha]$}
                        \State $p \gets \BP_{k}(n,m)$
		                \State $x_k \gets$ $ \prod\left(x_{k}, W_{p}^q(s_k)\right)$ 
		            \EndFor
              \State $\Bx(n) \gets \Bx(n) + \Bv_{k}x_{k}$
		        \EndFor
		    \EndIf
            \State Transmit $\Bx(n)$
		\EndFor
		\EndProcedure
	\end{algorithmic}
	\label{Alg:Delivery_main}
\end{algorithm}

\begin{exmp}
\label{exmp:interference-free-delivery}
Consider the network in Example~\ref{exmp:virt_network}. Based on $\CM_1$-$\CM_4$, the RIS of each user is $\CN_1 = \{4, 5, 6, 7, 8, 9, 10, 11, 12\}, \, \CN_2 = \{3,4\}, \, \CN_3 = \{4\}$ and $\CN_4 = \{1,2\}$. Note that there is a difference in the size and the number of subfiles needed by each user. Now, based on $\hat{Q}$, the corresponding DIS of each user is $\Check{\CN}_{{1}} = \{4, 5, 6, 7, 8, 9, 10, 11, 12\}, \, \Check{\CN}_{{2}} = \{1,2,3,7,8,9,10,11,12\}, \, \Check{\CN}_{{3}} = \{1,2,3,4,5,6,10,11,12\}$ and $\Check{\CN}_{{4}} = \{1,2,3,4,5,6,7,8,9\}$. Based on the delivery procedure, the requested subfiles of user $k$ are divided into $D_k$ file-fragments, where $D_1 = 2$, $D_2 = D_4 = 9$, $D_3 = 18$, and $\alpha$ is equal to $2$. It is clear that there exist $D_T = D_k(|\CN_k|) = 18$ file-fragments to be transmitted to each user. Based on~\eqref{virtual_index_replacement}, each virtual subfile is replaced by $\alpha$ actual missing file-fragments. As a result, the size of the transmitted data intended for user $1,2,3$ and $4$ are equal to $\frac{1}{12}, \frac{1}{18}, \frac{1}{36}$ and $\frac{1}{18}$ data units, respectively. Note that the size of the intended data for each user is proportional to the approximated rate of its location.

Now, let us review how the downlink message $\Bx(n)$ is built from $\Check{\Bx}(n)$. First, we form the FM matrices $\BG_1$-$\BG_4$ to map the RISs $\{\CN_k, \forall k \in [K]\}$ in to their corresponding DISs, i.e., $\{\Check{\CN}_{k}, \forall k \in [K]\}$. One such set of matrices is as follows
\begin{equation*} 
    \begin{aligned}
    \BG_1 = \begin{psmallmatrix}
    0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 0 & 0 \\
    0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 0 \\
    0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2
    \end{psmallmatrix},
    \BG_2 = \begin{psmallmatrix}
    0 & 0 & 0 & 2 \\
    0 & 0 & 0 & 2 \\
    0 & 0 & 0 & 2 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 2 & 0 \\
    0 & 0 & 2 & 0 \\
    0 & 0 & 2 & 0 \\
    0 & 0 & 0 & 2 \\
    0 & 0 & 2 & 0 \\
    0 & 0 & 1 & 1 
    \end{psmallmatrix},
    \BG_3 = \begin{psmallmatrix}
    0 & 0 & 0 & 2 \\
    0 & 0 & 0 & 2 \\
    0 & 0 & 0 & 2 \\
    0 & 0 & 0 & 2 \\
    0 & 0 & 0 & 2 \\
    0 & 0 & 0 & 2 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 2 \\
    0 & 0 & 0 & 2 \\
    0 & 0 & 0 & 2
    \end{psmallmatrix},
    \BG_4 = \begin{psmallmatrix}
    2 & 0 & 0 & 0 \\
    2 & 0 & 0 & 0 \\
    2 & 0 & 0 & 0 \\
    0 & 2 & 0 & 0 \\
    1 & 1 & 0 & 0 \\
    2 & 0 & 0 & 0 \\
    0 & 2 & 0 & 0 \\
    0 & 2 & 0 & 0 \\
    0 & 2 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 
    \end{psmallmatrix}.
    \end{aligned}
\end{equation*}
Accordingly, based on FM matrices and Algorithm~\ref{alg:File_ind_gen}, the \emph{file-fragment index matrix} $\BP_k$ are built as follows
\begin{equation*} 
    \begin{aligned}
    \BP_1 = \begin{psmallmatrix}
    4 & 4  \\
    7 & 7  \\
    10 & 10 \\
    0 & 0 \\
    5 & 5  \\
    6 & 6  \\
    8 & 8  \\
    9 & 9  \\
    0 & 0  \\
    11 & 11  \\
    0 & 0  \\
    12 & 12  
    \end{psmallmatrix},
    \BP_2 = \begin{psmallmatrix}
    4 & 4  \\
    0 & 0  \\
    4 & 4 \\
    3 & 3 \\
    3 & 4  \\
    4 & 4  \\
    0 & 0  \\
    3 & 3  \\
    3 & 3  \\
    4 & 4  \\
    3 & 3  \\
    0 & 0 
    \end{psmallmatrix},
    \BP_3 = \begin{psmallmatrix}
    4 & 4  \\
    4 & 4  \\
    0 & 0 \\
    4 & 4 \\
    0 & 0  \\
    4 & 4  \\
    4 & 4  \\
    4 & 4  \\
    4 & 4  \\
    0 & 0  \\
    4 & 4  \\
    4 & 4
    \end{psmallmatrix},
    \BP_4 = \begin{psmallmatrix}
    0 & 0  \\
    1 & 1  \\
    1 & 1 \\
    2 & 2 \\
    2 & 1  \\
    0 & 0  \\
    2 & 2  \\
    0 & 0  \\
    2 & 2  \\
    1 & 1  \\
    1 & 1  \\
    2 & 2
    \end{psmallmatrix}.
    \end{aligned}
\end{equation*}
Therefore, based on \emph{file-fragment index matrix} $\BP_k$ and equation~\eqref{eq:original data vector}, the first transmissions is
\begin{equation*} %\label{eq:first_transmission}
    \Bx(1) = \Bv_{1} \prod(A_{4}^{1}, A_{4}^{2}) +  \Bv_{2} \prod(B_{4}^{1}, B_{4}^{2}) +  \Bv_{3}\prod(C_{4}^{1}, C_{4}^{2}) \; ,
\end{equation*}
where $\prod(A, B)$ denotes the bit wise concatenation of file-fragments $A$ and $B$. Note that $\BP_k(n,m) = 0$ means there is no transmission for user $k \in [K]$ in time-slot $n\in \hat{N}$. Then, the corresponding received signal at user $1$ is 
\begin{equation*}
%\label{eq:first_reception}
\begin{aligned}
 y_1 = &\prod(A_{4}^{1}, A_{4}^{2})\Bh_1^H\Bv_{1}  + \underline{\prod(B_{4}^{1}, B_{4}^{2})}\Bh_1^H\Bv_{2} 
 +\underline{\prod(C_{4}^{1}, C_{4}^{2})}\Bh_1^H\Bv_{3} + w_1, 
\end{aligned}
\end{equation*}
where $w_1 \equiv z_1$ denotes the receiver noise at user $1$. 

Recall that files $B$ and $C$ correspond to the content of states $2$ and $3$. Therefore, based on the MLPDAs $\BQ_2$ and $\BQ_3$, subfiles $B_4$ and $C_4$ are available in the cache memory of user $1$. Hence, by estimating $\Bh_1^{H} \Bv_{k}, k \in \{2,3\}$, the underlined terms can be removed from the received signal and $\prod(A_{4}^{1}, A_{4}^{2})$ can be decoded interference-free. Moreover, the received signal at users $2$ and $3$ are as follows
\begin{equation*}
\begin{aligned}
        y_2 &=  \prod(B_{4}^{1}, B_{4}^{2}) \Bh_2^H \Bv_{2} + \underline{\prod(A_{4}^{1}, A_{4}^{2})} \Bh_2^H \Bv_{1} + w_2 \; , \\
        y_3 &= \prod(C_{4}^{1}, C_{4}^{2}) \Bh_3^H \Bv_{3} + w_3 \; , 
\end{aligned}
\end{equation*}
where $w_2 \equiv \Bh_2^H \Bv_{3}\prod(C_{4}^{1}, C_{4}^{2})+z_2$ and $w_3 \equiv \Bh_3^H(\Bv_{1} \prod(A_{4}^{1}, A_{4}^{2}) +  \Bv_{2} \prod(B_{4}^{1}, B_{4}^{2}))+z_3$ contain the (suppressed) interference terms plus noise at users $2$ and $3$, respectively.
Following a similar argument as above, users $2$ and $3$ can decode their intended data interference-free. The rest of the transmitted messages can be created following similar steps. Note that compared to conventional works~\cite{MLPDA_ISIT2022,lampiris2018adding,salehi2020lowcomplexity}, in all these transmissions, we allocate higher data transmission rates to user $1$ ($1.5$ times) and lower rates to user $3$ (half a time) than those assigned to users $2$ and $4$.
%However, due to the lack of the space the details are omitted.%The rest of the transmitted messages in the first phase can be similarly created as follows
%\begin{equation*} \label{eq:second&third transmissions}
%\begin{aligned}
%    \Bx(2) &= \Bv_{\{1,3\}}[A_{3}^{1} \ A_{3}^{2}] +  \Bv_{\{3,1\}} [C_{4}^{3} \ C_{4}^{4}] +  \Bv_{\{4,1\}}[D_{1}^{1} \ D_{1}^{2}] \; , \\
%    \Bx(3) &= \Bv_{\{1,4\}}[A_{4}^{1} \ A_{4}^{2}] +  \Bv_{\{4,1\}} [D_{1}^{3} \ D_{1}^{4}] +  \Bv_{\{2,1\}}[B_{4}^{3} \ B_{4}^{4}] \; ,
%\end{aligned}
%\end{equation*}
%Now, for the forth transmission, which corresponds to the first row of $\BC_2$, we target users $2,3$ and $4$. Based on the first row of $\BR_2$, the intended file-index for user $2$ is $\{3\}$, which corresponds to the third row of $\BF_2$. The only non-zero element in this row is $f_{3,3,2} = 6$. Similarly, the intended file-index for user $3$ is $\{2\}$, where the only non-zero element of the second row of $\BF_3$ is $f_{2,4,3} = 6$. Similarly, the intended file-index for user $4$ is $\{2\}$, which corresponds to the second row of $\BF_4$. However, in this case, there are two non-zero elements  $f_{2,1,4} = 3$ and $ f_{2,2,4} = 3$, which indicates that there exist two sets of candidate file-chunks to be transmitted to user $4$. Following Algorithm~\ref{alg:delivery_main}, the intended message for user $4$ is $Y_{\{2\}, 4} = \textsc{Concat} (D^{5}_{1}, D^{6}_{1})$. Hence, the first transmitted message in the second phase can be expressed as follows
%\begin{equation} \label{eq: forth transmission}
%    \Bx(4) = \Bv_{\{2,4\}}[B_{3}^{1} \ B_{3}^{2}] +  \Bv_{\{3,2\}} [C_{4}^{5} \ C_{4}^{6}] +  \Bv_{\{4,2\}}[D_{1}^{5} \ D_{1}^{6}].
%\end{equation}
%At this point, since the transmitted file-chunks in \eqref{eq: forth transmission} are based on matrix elements $f_{3,3,2}, f_{2,4,3}$ and $f_{2,1,4}$, these elements should be subtracted by two. Thus, at the end of $4$'th transmission, matrix elements $f_{3,3,2}, f_{2,4,3}$ and $f_{2,1,4}$, would be equal to $4,4$ and $1$, respectively. Now, in the second transmission of phase $2$, we target users $2$, $4$, and $1$. Based on the DP and MF matrices, only one file-chunk candidate for users $1$ and $2$. However, for user $4$ there exist two candidates $\{D^{v_4}_{1}, v_4 \in [9]\}$ and $ \{D^{v_4}_{2}, v_4 \in [9]\}$. Moreover, since at this point $f_{2,1,4}$ is equal to $1$, only one file chunk can be chosen from $D^{v_4}_{1}$ for this transmission, and the other one must be chosen from $D^{v_4}_{2}$. As the result, the intended message for user $4$ for the fifth transmission is generated as $Y_{\{2\}, 4} = \textsc{Concat} (D^{7}_{1}, D^{1}_{2})$. Therefore, following similar steps, the rest of the transmitted messages can be created similarly. However, due to the lack of space we have omitted the details. %as follows
%\begin{equation}
%    \begin{aligned}
%    \Bx(5) &= \Bv_{\{2,4\}}[B_{3}^{3} \ B_{3}^{4}] +  \Bv_{\{4,2\}}[D_{1}^{7} \ D_{2}^{1}] +  \Bv_{\{1,2\}}[A_{2}^{3} \ A_{2}^{4}] \; , \\
%    \Bx(6) &= \Bv_{\{2,1\}}[B_{4}^{5} \ B_{4}^{6}] +  \Bv_{\{1,2\}}[A_{2}^{5} \ A_{2}^{6}] +  \Bv_{\{3,2\}} [C_{4}^{7} \ C_{4}^{8}] \; , \\
%    \Bx(7) &= \Bv_{\{3,4\}}[C_{4}^{9} \ C_{4}^{10}]  +  \Bv_{\{4,3\}} [D_{2}^{2} \ D_{2}^{3}] +  \Bv_{\{1,3\}}[A_{3}^{3} \ A_{3}^{4}] \; , \\
%    \Bx(8) &= \Bv_{\{3,1\}}[C_{4}^{11} \ C_{4}^{12}] +  \Bv_{\{1,3\}}[A_{3}^{5} \ A_{3}^{6}] +  \Bv_{\{2,3\}}[B_{3}^{5} \ B_{3}^{6}] \; , \\
%    \Bx(9) &= \Bv_{\{3,2\}} [C_{4}^{13} \ C_{4}^{14}] +  \Bv_{\{2,3\}}[B_{3}^{7} \ B_{3}^{8}] +  \Bv_{\{4,3\}} [D_{2}^{4} \ D_{2}^{5}] \; , \\
%    \Bx(10) &= \Bv_{\{4,1\}} [D_{1}^{8} \ D_{1}^{9}] +  \Bv_{\{1,4\}}[A_{3}^{3} \ A_{4}^{4}] +  \Bv_{\{2,4\}}[B_{3}^{9} \ B_{4}^{7}] \; , \\
%    \Bx(11) &= \Bv_{\{4,2\}}[D_{2}^{6} \ D_{2}^{7}] +  \Bv_{\{2,4\}}[B_{4}^{8} \ B_{4}^{9}] +  \Bv_{\{3,4\}}[C_{4}^{15} \ C_{4}^{16}] \; , \\
%    \Bx(12) &= \Bv_{\{4,3\}} [D_{2}^{8} \ D_{2}^{9}] +  \Bv_{\{3,4\}}[C_{4}^{17} \ C_{4}^{18}] +  \Bv_{\{1,4\}}[A_{4}^{5} \ A_{4}^{6}] \; . \\
%    \end{aligned}
%\end{equation}
%Note that all these transmissions can be decoded interference-free following the same argument as in~\eqref{eq:first_reception} and~\eqref{eq:second&third transmissions}.
\end{exmp}
%
% \begin{thm}
% Every user receives its requested data using the proposed cache placement and content delivery algorithms.
% \end{thm}
% \begin{proof}
% A user $k \in \CK$ needs a total amount of $K$ sub-files to reconstruct its requested file $W(s_k)$. Assuming the user is in state $s_k$, $t_k$ sub-files are available in its cache memory. Hence, it needs to receive $K-t_k$ sub-files from the server. Based on the delivery scheme, each user is served by $K-\hat{t}$ virtual file-indexes $ I \in \CI_k$ and based on condition~\eqref{cond: total-delivery-chunk}, each virtual file-index $ I \in \CI_k$ delivers $\alpha(\hat{t}+L)$ file-chunks. As a result, $D_{\text{T}} = \alpha(\hat{t}+L)(K-\hat{t})$ file-chunks will be delivered to each user $k \in [K]$. Moreover, based on condition~\eqref{cond: total-file-chunk}, $D_k = \frac{\alpha(\hat{t}+L)(K-\hat{t})}{K-t_k}$ file-chunks belong to a single sub-file with index $j \in \CN_k$. Thus, $\frac{D_{\text{T}}}{D_k} = K-t_k$ sub-files are delivered to user $k$ during $K$ phases, and the proof is complete.
% \end{proof}
%
% \begin{thm}
% Using the proposed delivery algorithm, $\hat{t}+L$ users can be served interference-free in each transmission interval.
% \end{thm}
% \begin{proof}
% Based on the proposed delivery scheme, a set of $\hat{t}+L$ users determined by the $q$'th row of $\BC_p$ are targeted by the server for the $q$'th transmission of the $p$'th phase. Let us denote such a user set by $\CR_{\{q,p\}}$. Next, for proper data transmission, a virtual file-index $ I \in \CI_k$ will be allocated to user $k \in \CR_{\{q,p\}}$ based on the $q$'th row of matrix $_p$. Based on condition~\eqref{cond: feasibility} in Appendix~\ref{sec: Appendix A}, the transmitted content to user $k \in \CR_{\{q,p\}}$ can be cached out by all the users $ u \in \hat{\CT}_i$, where $\{\hat{\CT}_i \subseteq \CR_{\{q,p\}}, |\hat{\CT}_i| = \hat{t}\}$. As a result, the transmitted content needs to be suppressed for $\hat{t}+L - |\hat{\CT}_I | - 1 = L- 1$ other users through the beamforming, which requires $L$ antenna elements, and the proof is complete.
%
%On the other hand, based on the $q$'th row of the matrix $_p$, user $k \in \CR_{\{q,p\}}$ will receive some content, which all the users should cache out $u \in \hat{\CT}_i$ ($\hat{\CT}_I \subseteq \CR_{\{q,p\}}$) [MJ TWC], where $ I \in \CI_k$ is determined by $_p$. Note that this is guaranteed by condition~\eqref{cond: feasibility} in Appendix~\ref{sec: Appendix A}. 
% \end{proof}
%
\subsection{Weighted Max-Min Beamforming} \label{Sec:beamforming}

In this section, we discuss how the precoding vectors
%The precoder vectors 
$\Bv_{k}$ in~\eqref{eq: multiplexed signal}
should be designed optimally to improve the finite-SNR performance.
%are optimally designed in this section. 
%We propose a multi-rate transmission scheme, making 
The multi-rate transmission requirement of the proposed scheme in this paper makes
the beamformer design of conventional CC schemes (c.f.,~\cite{tolli2017multi,salehi2020lowcomplexity,D2D_CC_mahmoodi_2022}) inapplicable.
%for the proposed setting. 
To solve this issue, we alter the max-min-fairness beamforming in~\cite{salehi2020lowcomplexity} to a weighted-max-min (WMM) problem, where the weights reflect the non-uniform amounts of data transmitted to different users. 

%In the following, we review the delivery process and calculate the signal-to-interference-plus-noise-ratio (SINR) at the receivers to formulate the WMM problem.

As discussed in Section~\ref{sec:delivery}, the proposed scheme serves all the users using $\hat{N}$ transmission vectors $\Bx(n)$. Every vector $\Bx(n)$ comprises $|\CU(n)|$ data terms $x_{k}$ and the same number of beamforming vectors $\Bv_{k}$ as represented in~\eqref{eq:recieved_signal_sysmodel}. Hence, the corresponding received signal at user $k$ in $n$'th transmission can be rewritten as
\begin{equation} \label{eq:received_signal} 
    y_{k} = \Bh_{k}^{H}\Bv_{k}x_{k} + \sum_{\substack{i \in \CU(n) \\  k \in \CI_{i}(n) }}\Bh_{k}^{H}\Bv_{i}x_{i} + \sum_{\substack{j \in \CU(n) \\   k \notin \CI_{j}(n)}}\underline{\Bh_{k}^{H}\Bv_{j}x_{j}}+ z_k,
\end{equation}
where, each intended message $x_k$ contains a fresh data  for user $k$ with size 
\begin{equation} 
    c_k \equiv \frac{\alpha }{ F_{s_k} \alpha  (\frac{\hat{F}-\hat{Z}}{F_{s_k}-Z_{s_k}})} = \frac{1-m_k}{\hat{F}-\hat{Z}}.
\end{equation}
Recall that $x_{k}$ comprises $\alpha$ file-segments, where each segment is $\frac{1}{D_k}$ of a subfile and each subfile is $\frac{1}{F_{s_k}}$ data units in size. Note that the underlined terms in~\eqref{eq:received_signal} are removed from the received signals using cache memories (prior to the decoding procedure); hence, they are not considered interference. Accordingly, the received SINR at user $k$ is calculated as follows
\begin{equation}\label{eq:received_SINR}
    \gamma_k = \frac{|\Bh_{k}^{H}\Bv_{k}|^2}{\underset{{\substack{i \in \CU(n) : k \in \CI_{i}(n) }}}{\sum}|\Bh_{k}^{H}\Bv_{i}|^2+ N_0} .
\end{equation}
Moreover, the required time to deliver $x_k$ is calculated as $T_k = \frac{c_k}{\log (1 + \gamma_k)}$. Thus, the total delivery time to send $\Bx(n)$ is $T_{\CU(n)} = \max_{k \in \CU(n)}T_k$ [seconds]. 

Now, since we aim to minimize the delivery time, the beamformer optimization problem is formulated as $\underset{\{\Bv_{k}\}}\min \ \underset{k \in \CU(n)}\max \ T_{k}$, or equivalently as $\underset{\{\Bv_{k}\}}\max \ \underset{k \in \CU(n)}\min \ \frac{1}{c_k}\log(1 + \gamma_k)$, where $\log(1 + \gamma_k)$ is the dedicated rate to user $k$. Hence, the weighted minimum rate maximization for a given transmission $\Bx_{\CU(n)}$ can be formulated as follows
\begin{equation} 
\begin{array} {l}
	\label{opt:nonconvex_WMMF_basic}
		\underset{\{\Bv_{k}, \gamma_k\}}\max \ \underset{k \in \CU(n)}\min  \ 
	
        \frac{1}{c_k}\log(1 + \gamma_k)
	\\
	 \textrm{s.t.} \\ \quad
  \gamma_k \leq \frac{|\Bh_{k}^{H}\Bv_{k}|^2}{\underset{{\substack{i \in \CU(n) : k \in \CI_{i}(n) }}}{\sum}|\Bh_{k}^{H}\Bv_{i}|^2+ N_0}, \quad \forall k \in \CU(n), \\ \quad
	  \sum_{k \in \CU(n)}\|\Bv_{k}\|^2\leq P_T, 
\end{array}
\end{equation} 
where $P_T$ is the total transmit power at the transmitter. equation~\eqref{opt:nonconvex_WMMF_basic} can be rewritten as the following equivalent epigraph form
\begin{equation} \label{opt:nonconvex_WMMF_epic}
\begin{array} {l}
		\underset{\{\Bv_{k}, \bar{\gamma}, \gamma_k\}}\max \ \bar{\gamma}  \\
	 \textrm{s.t.}  \\ \quad
  \bar{\gamma} \leq \frac{1}{c_k}\log(1 + \gamma_k), \quad \forall k \in \CU(n), \\ \quad
  \gamma_k \leq \frac{|\Bh_{k}^{H}\Bv_{k}|^2}{\underset{{\substack{i \in \CU(n) : k \in \CI_{i}(n) }}}{\sum}|\Bh_{k}^{H}\Bv_{i}|^2+ N_0}, \quad \forall k \in \CU(n), \\ \quad
	  \sum_{k \in \CU(n)}\|\Bv_{k}\|^2\leq P_T. 
\end{array}
\end{equation} 
Constraint $\bar{\gamma} \leq \frac{1}{c_k}\log(1 + \gamma_k)$ can be equivalently expressed as $\exp(\bar{\gamma}) \leq (1+\gamma_k)^{\frac{1}{c_k}}$ as the exponential function is monotonically increasing. Finally, equation~\eqref{opt:nonconvex_WMMF_epic} can be equivalently expressed as follows
\begin{equation} \label{opt:nonconvex_WMMF_epic_MJ}
\begin{array} {l}
		\underset{\{\Bv_{k}, {\gamma}, \gamma_k\}}\max \ {\gamma}  \\
	 \textrm{s.t.}  \\ \quad
  \gamma^{c_{k}}-1 \leq \gamma_k, \quad \forall k \in \CU(n), \\ \quad
  \gamma_k \leq \frac{|\Bh_{k}^{H}\Bv_{k}|^2}{\underset{{\substack{i \in \CU(n) : k \in \CI_{i}(n) }}}{\sum}|\Bh_{k}^{H}\Bv_{i}|^2+ N_0}, \quad \forall k \in \CU(n), \\ \quad
	  \sum_{k \in \CU(n)}\|\Bv_{k}\|^2\leq P_T, 
\end{array}
\end{equation} 
where, $\gamma = \exp{(\bar{\gamma})}$. Now, quasi-convex problem~\eqref{opt:nonconvex_WMMF_epic_MJ} is the same as the one in~\cite{salehi2020lowcomplexity} with extra convex constraints $\gamma^{c_{k}}-1 \leq \gamma_k, \ \forall k \in \CU(n)$~\footnote{Note that $\gamma^{c_{k}}$ is convex for $c_k \geq 1$. Since $\{c_k\}$ are just considered as weights for rate allocation purposes, they can be easily replaced by $\{c_k \gets {c_k}/{\min_{k \in [K]} c_k}\}$ to make $\gamma^{c_{k}}$ a convex function.} and can be optimally solved using the Lagrangian duality (LD) scheme in~\cite{salehi2020lowcomplexity}%~\footnote{The LD procedure is presented in the context of \textit{uplink-downlink duality (UDD)} in~\cite{salehi2020lowcomplexity}.}. 

The LD scheme is an iterative fast-beamforming method used for linear-beamformer design in the literature (c.f.,~\cite{salehi2020lowcomplexity} and the references therein). Since it has already been thoroughly illustrated in~\cite{salehi2020lowcomplexity}, we will briefly review the LD scheme and its modifications for our WMM optimization. To this end, we first define $|\CU(n)|$ dual normalized beamforming vectors $\Bv^{\text{dual}}_{k}$ and their corresponding allocated power $\nu_k$, where LD necessitates
\begin{equation*}
    \sum_{k \in \CU(n)}\nu_k \|\Bv^{\text{dual}}_{k}\|^2 = \sum_{k \in \CU(n)}\|\Bv_{k}\|^2 .
\end{equation*}
For a given set of $\{\nu_k \ | \ k \in \CU(n) \}$, the dual vectors $\Bv^{\text{dual}}_{k}$ are given in a closed-form as follows
\begin{equation}\label{eq:dual_vectors}
    \Bv^{\text{dual}}_{k} = \frac{\left(\underset{{\hat{k} \in \CU(n): \hat{k} \in \CI_k(n) }}{\sum}\nu_{\hat{k}} \Bh_{\hat{k}}\Bh^{H}_{\hat{k}}+N_0\BI\right)^{-1}\Bh_k}{\left|\left(\underset{{\hat{k} \in \CU(n): \hat{k} \in \CI_k(n) }}{\sum}\nu_{\hat{k}} \Bh_{\hat{k}}\Bh^{H}_{\hat{k}}+N_0\BI\right)^{-1}\Bh_k\right|}
\end{equation}
Then, for a given set of dual beamforming vectors and their dedicated powers, the dual received SINR is calculated as follows
\begin{equation}\label{eq:dual_SINR}
    \gamma^{\text{dual}}_k = \nu_k\Bh^{H}_k \left(\underset{{\hat{k} \in \CU(n): \hat{k} \in \CI_k(n) }}{\sum}\nu_{\hat{k}} \Bh_{\hat{k}}\Bh^{H}_{\hat{k}}+N_0\BI\right)^{-1}\Bh_k.
\end{equation}

Note that based on LD, the dual SINR $\gamma^{\text{dual}}_k$ calculated in~\eqref{eq:dual_SINR} and the actual downlink SINR $\gamma_k$ calculated in~\eqref{eq:received_SINR} must be the same. Thus, by fixing target SINR to $\gamma$, the set of $\nu_k$ that satisfies $\gamma_k = \gamma^{c_k}-1$ with the minimum transmit power can be iteratively calculated as 
\begin{equation}\label{eq:fual_powers}
    \nu_k (\tau) = \frac{\gamma_k}{\gamma^{\text{dual}}_k(\tau-1)}\nu_k (\tau-1) = \frac{\gamma^{c_k}-1}{\Bh^{H}_k \left(\underset{{\hat{k} \in \CU(n): \hat{k} \in \CI_k(n) }}{\sum}\nu_{\hat{k}}(\tau-1) \Bh_{\hat{k}}\Bh^{H}_{\hat{k}}+N_0\BI\right)^{-1}\Bh_k}.
\end{equation}
The standard interference function approach in~\cite{uplink_downlink_1995} can be employed to prove the convergence of the joint update method in~\eqref{eq:fual_powers}. After convergence, i.e., when $\gamma^{\text{dual}}_k(\tau) = \gamma^{c_k}-1$, the minimum required transmit power to satisfy $\gamma^{\text{dual}}_k$ (i.e., $\sum_{k \in \CU(n)} \nu_k$) is compared with the available transmit power $P_T$. Accordingly, the new target SINR $\gamma$ is set for the next round. Thus, using bisection over $\gamma$, the set of $\{\nu^{*}_k  \ | \ \sum_{k \in \CU(n)} \nu^{*}_k = P_T, \ \gamma^{\text{dual}}_k = \gamma^{c_k}-1\}$ can be iteratively computed. 

When $\nu^{*}_k$ is computed for every $k \in \CU(n)$, the set of optimal downlink beamformers is computed as $\Bv_{k} = p_k\Bv^{\text{dual}}_{k}$, where $p_k$ is the downlink power dedicated to beamformer $\Bv_{k}$ and $\Bv^{\text{dual}}_{k}$ is computed using $\{\nu^{*}_k\}$ in~\eqref{eq:dual_vectors}. To compute $\{p_k\}$, we first define a vector $\Ba = [a_1, \dots, a_{|\CU(n)|}]$ and a diagonal matrix $\BD$ whose elements are $a_1, \dots, a_{|\CU(n)|}$, where
\begin{equation}\label{eq: a_definition}
    a_{k} = \frac{\gamma_k}{(1+\gamma_k)|\Bh^{H}_{k}\Bv^{\text{dual}}_{k}|^2}, \quad \forall k \in \CU(n).
\end{equation}
Next, we define a $|\CU(n)| \times |\CU(n)|$ square matrix $\BB$ whose elements are defined as 
\begin{equation}\label{b_definition}
    \BB(i,j) = \begin{cases} |\Bh^{H}_{i}\Bv^{\text{dual}}_{j}|^2 &\mbox{if } i \in \CI_j(n) \\
|\Bh^{H}_{i}\Bv^{\text{dual}}_{i}|^2 & \mbox{if } i = j \\
0 & \text{otherwise} 
\end{cases}.
\end{equation}
Finally, the downlink transmit power vector $\Bp = [p_1, \dots, p_{|\CU(n)|}]$ is  given in the following closed-form
\begin{equation}\label{p_definition}
    \Bp = N_0(\BI-\BD\BB)^{-1}\Ba.
\end{equation}
\begin{remark}\label{remark_proportional_rate}
    Similar to~\cite{mahmoodi2022asymmetric_arxiv_TWC2023}, the proposed WMM beamforming in~\eqref{opt:nonconvex_WMMF_epic_MJ} results in proportional rate allocation such that $\frac{\log(1+\gamma_k)}{\log(1+\gamma_{\bar{k}})} = \frac{c_{\bar{k}}}{c_{k}}$, $\forall(k,\bar{k}) \in \CU(n)$ . However, unlike~\cite{mahmoodi2022asymmetric_arxiv_TWC2023}, which requires non-linear receiver processing (SIC), the proposed beamforming solution in~\eqref{eq:dual_vectors}-\eqref{p_definition} is linear. Herein, the linear beamforming is enabled due to condition C3 in Definition~\ref{MLPDA_definition_new}, which prevents multiple messages transmission to a single user in each time instant. Due to the simplified beamforming procedure, the MLPDA-based scheme is more suitable for large networks .   
\end{remark}

It is easy to see that the total transmission time $T_T$ for the whole delivery process can be calculated as
\begin{equation}\label{eq:T_T_exact}
    T_T = \sum_{n \in [\hat{N}]}\max_{k \in \CU(n)}\frac{c_k}{\log(1+\gamma_k)} = \frac{1}{\hat{F}-\hat{Z}}\sum_{n \in [\hat{N}]}\max_{k \in \CU(n)}\frac{1-m_k}{\log(1+\gamma_k)}.
\end{equation}
Note that the total transmission time $T_T$ in~\eqref{eq:T_T_exact} can only be computed when the beamformers for all $\hat{N}$ transmissions are known, requiring user location and channel knowledge. However, actual user locations and channel states are unknown during the placement phase, making calculating $T_T$ impossible. Thus, for the placement phase in Section~\ref{sec:cache_placement}, we used an approximation of $T_T$ assuming uniform access probability for all the STUs as follows. 
\begin{lemma}\label{lemm:aprox_delivery_time}
The total delivery time $T_T$ calculated in~\eqref{eq:T_T_exact} can be approximated as
\begin{equation}\label{eq:T_T_approx}
    \hat{T}_T = \frac{K}{K\bar{m}+L}\max_{s \in \CS}\frac{1-m(s)}{r(s)} \; .
\end{equation}
\end{lemma}
\begin{proof}
We first substitute the term $log(1+\gamma_k)$ in~\eqref{eq:T_T_exact} with its upper bound $r(s_k)$ given in~\eqref{eq: state-rate} to get
\begin{equation}\label{eq:T_T-first_approx}
    T_T \sim \frac{1}{\hat{F}-\hat{Z}}\sum_{n \in [\hat{N}]}\max_{k \in \CU(n)}\frac{1-m_k}{r(s_k)} \; .
\end{equation}
Then, using inequality $\max\limits_{k \in {\CU(n)}}\frac{1-m(s_k)}{r(s_k)} \leq \max\limits_{s \in \CS}\frac{1-m(s)}{r(s)}$, we substitute the RHS of~\eqref{eq:T_T-first_approx} with its upper bound to get $T_T \sim 
\frac{\hat{N}}{\hat{F}-\hat{Z}}\max\limits_{s \in \CS}\frac{1-m(s)}{r(s)}$. Note that $\frac{\hat{N}}{\hat{F}-\hat{Z}} = \frac{K}{\frac{K(\hat{F}-\hat{Z})}{\hat{N}}}$, where $\frac{K(\hat{F}-\hat{Z})}{\hat{N}}$ is nothing but the sum-DoF~\cite{MLPDA_ISIT2022}. Hence, approximating $\frac{K(\hat{F}-\hat{Z})}{\hat{N}}$ with its upper bound $K\hat{m}+L$~\cite{MLPDA_ISIT2022}, we have 
\begin{equation}\label{T_T_approx_hat}
    T_T \sim \frac{K}{K\hat{m}+L}\max_{s \in \CS}\frac{1-m(s)}{r(s)} \; .
\end{equation}
Note that $\hat{m} = \min_{k \in [K]}m(s_k)$ requires user location knowledge, which is unknown during the placement phase. Thus, replacing $\hat{m}$ with its lower bound $\bar{m}$, \eqref{eq:T_T_approx} is achieved.
\end{proof}

Due to the location-dependent cache placement in~\eqref{cache-allocation}, the dedicated rate to each user is proportional to its transmitted data size (c.f., Remark~ \ref{remark_proportional_rate}). Hence, the delivery time is almost constant for any STU realization. Consequently, we can further simplify the delivery time approximation in~\eqref{T_T_approx_hat} by assuming $R_w =  \frac{r(s)}{1-m(s)}$ is independent of the STU $s$. As a result, we have $\hat{T}_T \sim \frac{K}{K\hat{m}+L} \frac{1}{R_w}$ and the symmetric rate will be $R_{w}^{s} = \frac{K}{T_T} = {(K\hat{m}+L)R_{w}}$. With a similar assumption, the symmetric rate of the conventional multi-antenna CC schemes (e.g.,~\cite{salehi2020lowcomplexity}) can also be approximated as $R_u^s = \frac{K}{T_T} = {(K\frac{M}{S}+L)R_u}$, where $R_{u} = \frac{\bar{r}}{1-M/S}$ and $\bar{r}$ is the standard max-min rate (c.f.~\cite{salehi2020lowcomplexity} Section~III-E). This results in
\begin{equation}\label{eq:rate_ratio}
    \frac{R^{{s}}_{{w}}}{R^{{s}}_{{u}}} = \frac{(K\hat{m}+L)R_{{w}}}{(K\frac{M}{S}+L)R_{{u}}},
\end{equation}
indicating that compared with the uniform cache placement schemes, the proposed location-dependent scheme can improve the delivery time if the DoF loss resulting from the non-uniform cache placement (i.e., $\frac{K\hat{m}+L}{K\frac{M}{S}+L}\leq 1$) can be compensated by the rate improvement (i.e., $\frac{R_{{w}}}{R_{{u}}} \geq 1$) due to the multi-rate transmission support.

% \subsection{Resolving the Imbalanced Allocated Memory Bottleneck}
% \label{Sec:phantom user}
% Our proposed location-dependent CC scheme simultaneously achieves $L$ spatial multiplexing gain and $\sim K\hat{m}$ coded caching gain while also addressing the wireless connectivity bottleneck problem. However, the $\min$ operation in $\hat{m}$ can wipe out the coded caching gain when a subset of users are located in states with strong wireless connectivity (i.e., a subset of users have small $m_k$ values). In other words, the performance improvement enabled by the underlying multi-antenna CC mechanism is limited by the users with better channel conditions, which is an undesired effect. To address this issue, we use the same \emph{phantom user} concept introduced in~\cite{mahmoodi2022asymmetric_arxiv_TWC2023}. For completeness, we briefly review the idea in the following. 

% Since users with strong wireless connectivity limit the coded caching gain, we can remove them from the CC-aided delivery phase. Then, the excluded users are substituted by the same number of phantom users, all located in poor-connectivity states (hence, with large $m_k$ values). In this regard, we assume phantom users to be part of the network when the transmission codewords are designed. However, these users will be ignored for the actual transmission. In other words, the data related to phantom users will not be included in the transmission vectors. This results in an improved global caching gain for users with poor channel conditions, as the $\min$ operation would no longer be limited to users with strong wireless connectivity. The strong users not served in the CC-aided delivery phase can be served separately through multi-user unicasting (i.e., considering spatial multiplexing and (possible) local caching gains only). As discussed in~\cite{salehi2021lowsubpacketization}, the DoF loss caused by phantom users can be (partly) compensated through an improved beamforming gain enabled by optimized beamformers.

% % \begin{algorithm}[t]
% % \small
% %     \caption{Phantom-based CC-Aided Delivery}
% % 	\begin{algorithmic}[1]
% % 		\Procedure{DELIVERY}{$\{\BQ_k\}$}
		
% % 		\State $k^{'} = \arg\min_{k \in \CK} m_k$
% % 		\If{$Km_{k^{'}} < Km_{\text{target}}$}\label{alg:limiting_user_elimination_start}
% % 		\State $\CK_p \gets \{ k \ | \ m(s_k) = m_{k^{'}} \}$
% % 		\If{$|\CK \setminus \CK_p| \geq Km_{k^{'}} + L$} \label{alg:phantom_remaining_user_check}
% % 		\State $k^{*} = \arg\min_{k \in \CK \setminus \CK_p} m_k$ \Else
% % 		\State $k^{*} \gets k^{'}$ \& $\CK_p \gets \emptyset$
% % 		\EndIf
% % 		\EndIf\label{alg:limiting_user_elimination_end}
% %             \State $\hat{\BQ} \gets \BQ_{k^{*}}$
% %             \ForAll{$k \in [K]$}
% %             \State Form $\BG_k$ based on $\hat{\BQ}$
% %             \State Compute $\BP_k$ based on $\BG_k$ using Algorithm~\ref{alg:File_ind_gen}
% %             \EndFor
% % 		\ForAll{$n \in [\hat{N}]$} %\label{alg:delivery_K_subsets}
% % 		\If{$|\CU(n) \setminus \CK_p| \geq L$} \label{alg:phantom_DoF_check}
% % 		\State $\Bx(n) \gets 0$
% % 		        \ForAll{$k \in \CU(n) \setminus \CK_p$}
% %                     \State $x_{k} \gets 0$
% % 		            \ForAll{$m \in [\alpha]$}
% %                         \State $p \gets \BP_{k}(n,m)$
% % 		                \State $x_k \gets$ $ \prod\left(x_{k}, W_{p}^q(s_k)\right)$ 
% % 		            \EndFor
% %               \State $\Bx(n) \gets \Bx(n) + \Bv_{k}x_{k}$
% % 		        \EndFor
% % 		    \EndIf
% %             \State Transmit $\Bx(n)$
% % 		\EndFor
% % 		\EndProcedure
% % 	\end{algorithmic}
% % 	\label{Alg:Delivery_phantom}
% % \end{algorithm}

% The phantom-based CC-aided content delivery is summarized in Algorithm~\ref{Alg:Delivery_phantom}. In this algorithm, we keep substituting users with best channel conditions with phantom users until the coded caching gain $K\hat{m}$ is favorable, i.e., larger than or equal to $Km_{\text{target}}$\footnote{In this paper, we have selected the $Km_{\text{target}}$ value by experimenting. Finding the optimal value for this parameter is left for future research.}. Moreover, we also check that the actual achievable DoF for the remaining users does \emph{not} fall below $Km_{k^{'}} + L$, which is the current achievable DoF. After CC-aided delivery, all the remaining data not served during this phase is transmitted in a traditional multi-user unicasting fashion. The following example clarifies this procedure.

% \begin{exmp}
% \label{exmp:interference-free-delivery_phant}
% Consider a similar setting as in Example~\ref{exmp:interference-free-delivery}, where users are now located such that $s_2 = s_3 = s_4 =3$, and $s_1 = 1$. Consequently, we have
% \begin{equation*} 
%     \begin{aligned}
%     \CM_1 = \{ A_{4}, A_{5}, A_{6}, A_{7}, A_{8}, A_{9}, A_{10}, A_{11}, A_{12} \}, \
%     \CM_2 = \{ B_{3}\}, \
%     \CM_3 = \{ C_{4}\}, \
%     \CM_4 = \{ D_1\}. 
%     \end{aligned}
% \end{equation*}
% Here, without phantom-based CC-aided procedure, the delivery is limited by user $1$. Consequently,  similar to Example~\ref{Alg:Delivery_phantom}, the delivery is carried out in twelve transmissions based on $\BQ_1$. However, following Algorithm~\ref{Alg:Delivery_phantom}, user $1$ is first excluded from the set of CC-aided users (i.e., $\CK_p = \{1\}$), and hence, the new common MLPDA is $\hat{\BQ} \equiv \BQ_3$. Thus, based on $\BQ_3$, the CC-aided data delivery is done in one transmission followed by a unicasting message as follows:
% \begin{equation}\nonumber 
%     \Bx(1) = \Bh_2B_{3}+\Bh_3C_{4}+\Bh_4D_{1},
% \end{equation}
% and 
% \begin{equation*}
%        \Bx(2) = \Bh_{1} \left(\prod( A_{4}, A_{5}, A_{6}, A_{7}, A_{8}, A_{9}, A_{10}, A_{11}, A_{12}\right).
% \end{equation*}
% Here, based on $\BQ_3$, $\CI_k = \emptyset, \forall k \in [K]$, so the optimal precoder for user $k$ is matched to its corresponding channel vector $\Bh_k$. As a result, the delivery time can potentially decrease due to reduced inter-message interference. 
% \end{exmp}

==> Sysmodel_old.tex <==
%!TeX root = d2d-cc.tex

\section{System Model}
\label{sec:sysmodel}
A system model similar to~\cite{mahmoodi2022asymmetric_arxiv_TWC2023} is explored here with new placement and transmission schemes, mainly focusing on a bounded environment such as a gaming hall, operating theater, or exhibition hall. In the considered system model, a server with $L$ antennas serves $K$ single-antenna users\footnote{The proposed system model can be easily extended to multi-antenna receivers following a similar approach proposed in~\cite{salehi2021lwsa}.} through wireless communication links. Each user is equipped with a finite-size memory and is free to move throughout the environment, and $\CK = [K]$ denotes the set of users. Users request the server for new data occasionally, and the requested data is assumed to depend on the users' locations and the application's requirements. As discussed in~\cite{mahmoodi2022asymmetric_arxiv_TWC2023}, the requested data content comprises static and dynamic parts (see Figure~\ref{fig:static_dynamic_decomposition}), and the detailed FoV is rendered by obtaining both parts. Though the static part usually forms a significant share of the FoV, the dynamic part is one of the main factors for a realistic perception. Hence, the dynamic part is continuously delivered parallel to the static part by allocating a portion of the available radio resources (frequency, time, space). 

Nevertheless, the dynamic part of the FoV is almost entirely cacheable in a typical virtual gaming scenario, for instance, by defining geometrical shapes, textures, and avatars. Hence, the end users can partially store the dynamic and static parts in advance, considering their available memory~\cite{flashback_2016_VR_static_dynamic_support}. However, low-overhead control data for reconstructing the dynamic content using both the cached elements and the multicast data must be provided to the users due to the interaction of the objects in the virtual world. We only focus on the wireless delivery of cachable content in this paper, which is partially aided by in-device memories. A wireless XR environment is an example of a real-world application of the described communication setup, where the requested data is required to reconstruct each user's location-dependent 3D FoV. In this regard, consider a 3-D gaming environment, where obstacles, walls, buildings, and surrounding nature are examples of the static part. On the other hand, players themselves and how they interact with the game are dynamic content examples. Considering the wireless connection nature, users in different locations experience dissimilar channel conditions. Therefore, this paper develops a cache-aided communication scheme to maximize the achievable rate over the wireless link and avoid excessive delivery times at wireless bottlenecks. 

Section~\ref{section:our_contribution} discussed how the application environment is divided into different STUs, and that each STU requires its scenery file. The scenery file is assumed to contain enough data to render the entire $360$-degree spherical FoV around the user. Whenever a user's head rotation or other environmental changes trigger a dynamic change, it is assumed that the FoV correction is locally done by the users based on the available sensory data or after the server has provided the necessary instructions for rebuilding the new content. We assume the STU mapping is performed such that every point in a given STU has almost the same level/quality of wireless connectivity. Figure~\ref{fig:system-model} represents a simple application environment with eight STUs, where $\CS$ denotes the set of STUs and $|\CS| = S$. Denote $W(s)$ as the file requested by a user in state $s \in \CS$ and, without loss of generality, assume $|W(s)| = F$ bits for every $s\in\CS$. A normalized data unit is considered in this paper if it is not stated otherwise, and $F$ is dropped in subsequent notations.

We follow a centralized data delivery process comprised of cache placement and content delivery phases. During the placement phase, each user $k$ equipped with a cache memory of $M$ (normalized) bits stores a message $Z_{k} = Z_{k}(W(s_{1}), \dots, W(s_{S}))$ in its cache, where $Z_{k}(\cdot)$ denotes a function of the files $W(s)$, $\forall s \in \CS$, with entropy not larger than $M$ bits. Then, during the delivery phase, a request vector $\Bd:= \{d_k \ | \ d_k \in \CS$, $\forall k \in \CK\}$ is first collected at the BS. Next, based on $\Bd$, the BS transmits several precoded messages $\Bx_{\CU}$ such that at the end of the transmission, all users can reliably recover their requested files. We use $\Bx_{\CU}$ to denote a message aimed at user set $\CU \subseteq \CK$ and assume that precoded messages $\Bx_{\CU}$ are transmitted at different intervals. Before going through a detailed discussion on the delivery process in Section~\ref{sec:delivery}, let us briefly review the transmit and receive signals in this section. Every message $\Bx_{\CU}$ comprises several unit power codewords $x_k$, where each codeword $x_k$ contains useful data for a user $k \in \CU$. Thus, $\Bx_{\CU}$ is built as
%\begin{equation}
$    \Bx_{\CU} = \sum_{k \in {\CU}} \Bv_{\CI_k}x_{k} $,
%\end{equation}
where $\Bv_{\CI_k} \in \mathbb{C}^{L}$ denotes the precoding vector dedicated to codeword $x_k$. 
%
After the transmission of $\Bx_{\CU}$, every user $k \in \CU$ receives
\begin{equation}\label{eq:recieved_signal_sysmodel}
    y_{k,\CU} = \Bh_{k,\CU}\herm\sum_{\bar{k} \in \CU}\Bv_{\CI_{\bar{k}}}x_{\bar{k}} + z_k,
\end{equation}
where the channel vector between the BS and user $k$ is denoted by $\Bh_{k,\CU} \in \mathbb{C}^{L}$, and $z_k \sim \mathbb{CN}(0,N_0)$ represents the additive white Gaussian noise.
Note that both the local cache content $Z_k$ and the received signals from the wireless channel over different time intervals (i.e., $y_{k,\CU}$) are used at the decoder of user $k$ to reproduce the requested file $W_{d_k}$. In the following, since the same procedure is repeated at each transmission, we present the delivery procedure for a specific transmission and use $y_{k}$ and $\Bh_k$ interchangeably with $y_{k,\CU}$ and $\Bh_{k,\CU}$. Moreover, the instantaneous channel state information is assumed to be perfectly known at the transmitter during the delivery phase, which is utilized for beamformer design and rate allocation.

Finally, as discussed in~\cite{mahmoodi2022asymmetric_arxiv_TWC2023}, a rate approximation is necessary for a proper location-dependent cache design during the placement phase. Note that, unlike the delivery phase, the actual rates can not be computed during the placement phase. During this phase, we are unaware of the delivery details, such as the number of users scheduled in parallel, all users' locations and channel states, and the precoding algorithms. The aim is to have a relative rate difference among different STUs to allocate distinct portions of memory accordingly. Intuitively, to avoid extensive transmission times for users with poor connectivity, data needed at STUs with the least approximated rates will occupy most of the memory. To this end, we use the following rate approximation as in~\cite{mahmoodi2022asymmetric_arxiv_TWC2023} 
%However, there is no knowledge about users' channel conditions during the placement phase. Thus, we need a prior estimate or prediction of the normalized achievable throughput $r(s)$ [files/second] at each state $s$ for the location-dependent cache placement phase. The expected location-specific data rates $r(s)$ can be attained through various means, e.g., collecting statistics from past active users. Since the proposed placement scheme in this paper is oblivious to the rate estimation method, we use a hypothetical single-user scenario to conveniently estimate the user's achievable rate at each state. Note that actual user-specific delivery rates depend on the number of users scheduled in parallel, precoding algorithms used, etc. As a result, the expected interference-free throughput attained in state $s\in \CS$, normalized by the file size $F$ [bits], can be roughly approximated as
\begin{equation} \label{eq: state-rate}
    {r}(s) = \frac{\Omega}{F}C_p\mathbb{E}\big[\log(1+\frac{P_T \ \|\Bh_{k_s}\|^2}{N_0})\big] \quad \text{[files/second]},
\end{equation}
where $C_p$ is a pre-log scaling factor containing any practical overhead, $P_T$ is the transmission power, $\Omega$ is the communication bandwidth, and $\Bh_{k_s} \in \mathbb{C}^{L}$ is the channel vector between the server and a user $k$ located in state $s$. Note that the expectation is taken over all user locations and channel realizations in state $s$ (c.f.,~\cite{mahmoodi2022asymmetric_arxiv_TWC2023} for more details). %It is worth noting that (2) is an `upper bound' for the achievable rate at any state. The main objective is to have a relative throughput measure among states. The scaling (including practical overheads, the impact of scheduling, etc.) would not change the memory allocation process since it can be considered almost the same across all the states. 

\begin{figure}
    \centering 
    \includegraphics[width=0.5\columnwidth,keepaspectratio]{figs/system model.pdf}
    \caption{An application environment with $K=3$ users, split into $S=8$ STUs. $r(j)$ is the state-specific achievable rate and $r(3) > r(2) > r(7)$. $X_{123}$ is the transmitted message, $X_i$ and ${\bf{w}}_i$ represents the data part intended for user $i$ and its corresponding precoder, respectively. The black bar below each user indicates how much of the requested data is cached.}
    \label{fig:system-model}
\end{figure}


==> figs/Data/Figrate.tex <==
States	rates	Memory
1	3	25
2	2	50
3	1	75
4	2	50
5	3	25


==> figs/Fig2.tex <==
%\begin{figure}
    \centering
    \resizebox{0.6\columnwidth}{!}{%

    \begin{tikzpicture}

    \begin{axis}
    [
    % put axis lines at left and bottom
    axis lines = left,
    % control axis labels
    xlabel near ticks,
    xlabel =  {States},
    ylabel =  {Rate [bits/Hz/s] \ref{rate}},
    ylabel near ticks,
    ymin = 0, %ymax = 20,
    % control legend position
    legend pos = north west,
    % control size of tick marks (10,20,30,etc)
    ticklabel style={font = \small},
    % control major grids
    grid=both,
    major grid style={line width=.2pt,draw=gray!30},
    % control minor grids
    %grid style={line width=.1pt, draw=gray!10},
    %minor tick num=5,
    %ybar interval=0.7,
    ]
    
    \addplot
    [mark = square, black]
    table[y=rates,x=States]{figs/Data/Figrate.tex};
    %\addlegendentry{\tiny rate}
    \label{rate}
    \end{axis}
    
    \begin{axis}
    [
    % put axis lines at left and bottom
    axis lines = right,
    axis x line*=bottom,
    xtick={},
    xticklabels={},
    axis y line*=right,
    % control axis labels
    %xlabel near ticks,
    %xlabel = \smaller {States},
    ylabel =  {Memory \%  \ref{memory}},
    ylabel near ticks,
    ymin = 0, ymax = 100,
    % control legend position
    %legend pos = north west,
    % control size of tick marks (10,20,30,etc)
    ticklabel style={font= \small},
    % control major grids
    %grid=both,
    major grid style={line width=.2pt,draw=gray!30},
    % control minor grids
    %grid style={line width=.1pt, draw=gray!10},
    %minor tick num=5,
    %ybar interval=0.7,
    ]
    
    \addplot
    [mark = x, gray]
    table[y=Memory,x=States]{figs/Data/Figrate.tex};
    %\addlegendentry{\tiny memory}
    \label{memory}
    \end{axis}

    \end{tikzpicture}
    }

    \caption{Location-specific rate and memory distributions for Example~\ref{exmp:placement}.
    }
    \label{fig:rate&cache_distribution}
%\end{figure}

==> figs/PlacementFigure.tex <==
\begin{figure}[ht]
    %\smaller
    \centering
    \resizebox{1\columnwidth}{!}{%
    \begin{tabular}{c}
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
            \cline{2-13}
            \multicolumn{1}{c|}{} & \multicolumn{12}{c|}{$\,\quad \quad W(s) \ \quad$} \\
            \hline
            \multirow{4}{*}{\rotatebox[origin=c]{90}{ $s=1,5$}} & \multicolumn{1}{c|}{\cellcolor{gray!50}} & \multicolumn{1}{c|}{\cellcolor{gray!50}} & \multicolumn{1}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 
            \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 
            \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & user $1$ \\
            \cline{2-14}
            & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  
            \multicolumn{1}{c|}{\cellcolor{gray!50}} & \multicolumn{1}{c|}{\cellcolor{gray!50}} & \multicolumn{1}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 
            \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & user $2$ \\
            \cline{2-14}
            & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 
            \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 
            \multicolumn{1}{c|}{\cellcolor{gray!50}} &  \multicolumn{1}{c|}{\cellcolor{gray!50}} &  \multicolumn{1}{c|}{\cellcolor{gray!50}} &  
            \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & user $3$ \\
            \cline{2-14}
            & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 
            \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 
            \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 
            \multicolumn{1}{c|}{\cellcolor{gray!50}} &  \multicolumn{1}{c|}{\cellcolor{gray!50}} &  \multicolumn{1}{c|}{\cellcolor{gray!50}} &  user $4$ \\
            \hline
            \multicolumn{14}{c}{}\\[-0.2em]
        \end{tabular} 
        % \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
        %     \cline{2-13}
        %     \multicolumn{1}{c|}{} & \multicolumn{12}{c|}{$ W(s) $} \\
        %     \hline
        %     \multirow{4}{*}{\rotatebox[origin=c]{90}{ $s=2,4$}} & \multicolumn{3}{c|c|c|c|}{\cellcolor{gray!50}} & 
        %     \multicolumn{3}{c|c|c|c|}{} & 
        %     \multicolumn{3}{c|c|c|c|}{} & 
        %     \multicolumn{3}{c|c|c|c|}{\cellcolor{gray!50}} & user $1$ \\
        %     \cline{2-14}
        %     & \multicolumn{3}{c|c|c|c|}{\cellcolor{gray!50}} & 
        %     \multicolumn{3}{c|c|c|c|}{\cellcolor{gray!50}} & 
        %     \multicolumn{3}{c|c|c|c|}{} & 
        %     \multicolumn{3}{c|c|c|c|}{} & user $2$ \\
        %     \cline{2-14}
        %     & \multicolumn{3}{c|c|c|c|}{} & 
        %     \multicolumn{3}{c|c|c|c|}{\cellcolor{gray!50}} & 
        %     \multicolumn{3}{c|c|c|c|}{\cellcolor{gray!50}} & 
        %     \multicolumn{3}{c|c|c|c|}{} & user $3$ \\
        %     \cline{2-14}
        %     & \multicolumn{3}{c|c|c|c|}{} & 
        %     \multicolumn{3}{c|c|c|c|}{} & 
        %     \multicolumn{3}{c|c|c|c|}{\cellcolor{gray!50}} & 
        %     \multicolumn{3}{c|c|c|c|}{\cellcolor{gray!50}} & user $4$ \\
        %     \hline
        %     \multicolumn{14}{c}{}\\[-0.2em]
        % \end{tabular} \\
                \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
            \cline{2-13}
            \multicolumn{1}{c|}{} & \multicolumn{12}{c|}{$\,\quad \quad W(s) \ \quad$} \\
            \hline
            \multirow{4}{*}{\rotatebox[origin=c]{90}{ $s=2,4$}} & \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\quad\quad\quad\quad} & 
            \multicolumn{3}{c|}{\quad\quad\quad\quad} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & user $1$ \\
            \cline{2-14}
            & \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\quad\quad\quad\quad} & 
            \multicolumn{3}{c|}{\quad\quad\quad\quad} & user $2$ \\
            \cline{2-14}
            & \multicolumn{3}{c|}{\ \quad\quad\quad\quad} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\ \quad\quad\quad\quad} & user $3$ \\
            \cline{2-14}
            & \multicolumn{3}{c|}{ \quad\quad\quad\quad} & 
            \multicolumn{3}{c|}{ \quad\quad\quad\quad} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & user $4$ \\
            \hline
            \multicolumn{14}{c}{}\\[-0.2em]
        \end{tabular} 
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
            \cline{2-13}
            \multicolumn{1}{c|}{} & \multicolumn{12}{c|}{$\,\quad \quad W(s) \ \quad$} \\
            \hline
            \multirow{4}{*}{\rotatebox[origin=c]{90}{ $s=3$}} & \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\quad\quad\quad\quad} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & user $1$ \\
            \cline{2-14}
            & \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\quad\quad\quad\quad} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & user $2$ \\
            \cline{2-14}
            & \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\ \quad\quad\quad\quad} & user $3$ \\
            \cline{2-14}
            & \multicolumn{3}{c|}{\ \quad\quad\quad\quad} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & user $4$ \\
            \hline
            \multicolumn{14}{c}{}\\[-0.2em]
        \end{tabular}
    \end{tabular}%
    }
    \caption{Cache placement visualization for Example~\ref{exmp:placement}. Gray cells show the available subfile in each user's cache, and the white ones are missing.}
    \label{fig:cache pool}
\end{figure}

==> intro_old.tex <==
\section{Introduction}
%The main contributor to global mobile traffic growth is the advent of various wireless devices with numerous features and capabilities in recent years. Currently, the majority of wireless devices are comprised of mobile flat screens, such as cell phones and tablets. However, the market is constantly flooded with new technologies and devices which can support data-intensive applications in different forms and capabilities, requiring even more traffic than before~\cite{cisco2020}. For instance, new data-hungry applications such as wireless extended reality (XR) are expected to be shortly established by the introduction of new wireless eyewears~\cite{Mahmoodi_immersive_isit2021,mahmoodi_ICC2022_nonsym,mahmoodi2022asymmetric, mahmoodi2022asymmetric_arxiv_TWC2023, salehi2022enhancing, flashback_2016_VR_static_dynamic_support}. 
Mobile traffic is exponentially growing, primarily due to the growing number of mobile devices, such as cell phones and tablets. Moreover, the market is constantly flooded with technologies and devices which can support new data-intensive applications in different forms and capabilities, requiring even more traffic than before~\cite{cisco2020}. Wireless eyewear, for example, will facilitate the development of unprecedented data-hungry applications, such as mobile extended reality (XR)~\cite{Mahmoodi_immersive_isit2021,mahmoodi_ICC2022_nonsym,mahmoodi2022asymmetric, mahmoodi2022asymmetric_arxiv_TWC2023, salehi2022enhancing, flashback_2016_VR_static_dynamic_support}. Wireless XR applications are in fact subject to strict quality of service (QoS) requirements including low latency ($ < 10$ ms), and high data rate transmission ($6.37 - 95.55$ Gbps)~\cite{Nokia-immersive,6G_white_paper_2020,bastug2017toward, taleb2022_towards_XR_vision, walid_sad_bennis_VR_XR_2022,wireless_virtual_reality_TCOM2018}. This differs greatly from conventional ultra-low latency and low-rate requirements for internet-of-things applications~\cite{URLLC_ICC_2017}. The low latency along with the high delivery rates require more sophisticated transmission methods than those offered by current wireless network standards~\cite{bastug2017toward, taleb2022_towards_XR_vision, walid_sad_bennis_VR_XR_2022}. Therefore, to meet the requirements of future wireless XR applications, a new 
scheme with a higher bandwidth efficiency is needed. %This contrasts the conventional low-rate ultra-low latency requirement in the internet of things applications~\cite{URLLC_ICC_2017}. In fact, the low latency with high-rate transmission calls for more intelligent transmission schemes than the one available with the current wireless network standards~\cite{bastug2017toward, taleb2022_towards_XR_vision, walid_sad_bennis_VR_XR_2022}. 

Furthermore, upcoming mobile broadband applications rely heavily on asynchronous content reuse~\cite{proactive_caching_Cm2016}, which allows proactive caching at the end-users to relieve network congestion and bandwidth consumption during peak times~\cite{role_of_caching_in_future_wireless_caire_JSAC2018}. In this regard, various studies have explored proactive caching in a single-input-single-output (SISO) configuration, demonstrating the role of cache placement for meeting XR application requirements~\cite{sun2019communications,yang2018communication,sun2020bandwidth,dang2019joint}. Specifically, with the available memory at the end users, the whole or part of the requested content can be cached beforehand and rendered by the end user at the request time. This results in significant bandwidth and delay-reduction gains and alleviates the traffic burden over the wireless network~\cite{sun2019communications,yang2018communication,sun2020bandwidth,dang2019joint}.  

Unlike conventional caching schemes, which rely on the available memory of each user (see, e.g.,~\cite{proactive_caching_Cm2016, role_of_caching_in_future_wireless_caire_JSAC2018, sun2019communications,yang2018communication,sun2020bandwidth,dang2019joint, bastug2014living,yang2015analysis}), the \ac{CC} scheme has been proposed to benefit from the aggregated memory throughout the network\cite{MaddahAli-2014}. Specifically, the CC scheme enjoys a so-called \textit{global caching} gain available through careful cache placement and multicast transmission, resulting in improved performance compared to traditional schemes~\cite{proactive_caching_Cm2016, role_of_caching_in_future_wireless_caire_JSAC2018, sun2019communications,yang2018communication,sun2020bandwidth,dang2019joint, bastug2014living,yang2015analysis}. As such, the transmission bandwidth for delay-constrained XR applications has been effectively reduced in a \ac{SISO} setup by leveraging coded cache placement and mobile device computing capabilities~\cite{CC_edge_computing_for_VR_twc2021}. Moreover, the CC scheme is especially advantageous for large networks because the global caching gain achieved via the CC scheme scales linearly with the number of users in the network. As such, the CC scheme is ideal for collaborative XR scenarios where a group of users is served simultaneously within a confined environment, with each user's individual choices and actions having an impact on the overall results perceived by all users (c.f.,~\cite{Mahmoodi_immersive_isit2021, mahmoodi2022asymmetric,mahmoodi_ICC2022_nonsym, mahmoodi2022asymmetric_arxiv_TWC2023, salehi2022enhancing}). In this regard, location-dependent CC-based cache placement and delivery schemes have been proposed in~\cite{Mahmoodi_immersive_isit2021}, specially tailored for a \ac{SISO} XR application.

In addition, the CC scheme's ability to combine global caching and spatial multiplexing gains is another critical feature~\cite{pooya-cc-physical-2019-journal}. This is particularly appealing given that multi-antenna connectivity will be a crucial feature of upcoming communication systems~\cite{6G_white_paper_2020}. Thus, the SISO setup in~\cite{Mahmoodi_immersive_isit2021} has been extended to a multiple-input single-output (MISO) setup in~\cite{ mahmoodi2022asymmetric,mahmoodi_ICC2022_nonsym, mahmoodi2022asymmetric_arxiv_TWC2023}, benefiting from multiplexing and global caching gains simultaneously. The current study extends our earlier works in~\cite{ mahmoodi2022asymmetric,mahmoodi_ICC2022_nonsym, mahmoodi2022asymmetric_arxiv_TWC2023} by using a simple transceiver design without the practical limitations of our earlier studies. By contrast with~\cite{ mahmoodi2022asymmetric} and~\cite{ mahmoodi2022asymmetric_arxiv_TWC2023}, the proposed method also applies to large networks and does not require a higher multiplexing gain than the coded caching gain required by~\cite{mahmoodi_ICC2022_nonsym}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Interference cancellation and multi-rate transmission with \ac{CC}}

\noindent\textbf{Bit-level coded caching.} 
The global caching gain in~\cite{MaddahAli-2014} is achieved by combining parts of several requested files to form a single message, enabling a multicast transmission to serve a group of users with a common message. Since, in~\cite{MaddahAli-2014}, the file parts are combined by applying an XOR operation on the file bits, it is called \emph{bit-level} coded caching in this paper. Following a similar data XORing approach, the original error-free framework in~\cite{MaddahAli-2014} was extended to more practical scenarios, including multi-server and wireless multi-antenna coded caching~\cite{Shariatpanahi2016,pooya-cc-physical-2019-journal,yu2017exact,tolli2017multi}. The early high \ac{SNR} analysis in~\cite{Shariatpanahi2016,pooya-cc-physical-2019-journal,yu2017exact} proved that the \ac{DoF} achieved by the CC scheme is optimal for uncoded cache placement and single-shot data delivery. Later on, the low-SNR analysis in~\cite{tolli2017multi} showed that an optimized multi-antenna precoder design is necessary for the CC scheme to achieve efficient performance in the low-SNR region. Soon, device-to-device (D2D) CC schemes were proposed (e.g.,~\cite{Ji2016,D2D-CC-Optload-memtradeof-caire-2019,D2D_CC_mahmoodi_2022}) to increase the network throughput. In this regard, an infrastructure-less network is studied in~\cite{Ji2016}, i.e., the only available link is D2D, where CC-based cache placement and delivery schemes were designed to achieve an optimal transmission rate~\cite{D2D-CC-Optload-memtradeof-caire-2019}. Later on, the system model in~\cite{Ji2016} and~~\cite{D2D-CC-Optload-memtradeof-caire-2019} was extended in~\cite{D2D_CC_mahmoodi_2022} to a general framework where D2D transmissions complemented downlink transmission.

While the CC schemes proposed in early studies~\cite{Shariatpanahi2016,pooya-cc-physical-2019-journal,yu2017exact,tolli2017multi,Ji2016,D2D-CC-Optload-memtradeof-caire-2019,D2D_CC_mahmoodi_2022} provide a significant performance boost, they also suffer several practical bottlenecks such as exponential file-division requirement. Hence, a combinatorial subfile assignment based on placement delivery array (PDA) is proposed in~\cite{PDA_first_2017} to reduce the subpacketization of the earlier studies. Interestingly, authors in~\cite{PDA_first_2017} showed that the scheme in~\cite{MaddahAli-2014} (as well as~\cite{Shariatpanahi2016,pooya-cc-physical-2019-journal,yu2017exact,tolli2017multi,Ji2016,D2D-CC-Optload-memtradeof-caire-2019,D2D_CC_mahmoodi_2022}) could also be presented as a PDA. Motivated by the generalized framework in~\cite{PDA_first_2017}, later studies, e.g.,~\cite{cheng_generalized_PDA_2019,DPDA2019,cheng_centralized_PDA_framework_2021}, proposed various PDA-based CC schemes for different settings, aiming for reduced file-division requirements. In fact, the proposed framework in~\cite{PDA_first_2017,cheng_generalized_PDA_2019,DPDA2019,cheng_centralized_PDA_framework_2021} translates the placement and delivery scheme design to a matrix formation based on proper predefined conditions.

\noindent\textbf{Signal-level coded caching.} 
Different from~\cite{PDA_first_2017,cheng_generalized_PDA_2019, DPDA2019,cheng_centralized_PDA_framework_2021}, the proposed scheme in~\cite{lampiris2018adding} benefits from the number of antennas at the transmitter to avoid excessive file division. Unlike~\cite{Shariatpanahi2016}, where the files were mixed using the XOR operation over different files' bits, the scheme in~\cite{lampiris2018adding} multiplexes different requested files over the air and is called \emph{signal-level} coded caching in this paper. Motivated by the proposed scheme in~\cite{lampiris2018adding}, authors in~\cite{Shahred_cache_Emanuele_2020} extend the system model in~\cite{lampiris2018adding} to a shared cache scenario, where a limited number of cache-enabled helper nodes serves a group of cache-less users. The centralized system model in~\cite{Shahred_cache_Emanuele_2020} was later extended to a decentralized scenario in~\cite{Shared_cache_decentrlized_2021}. Following a different technique, authors in~\cite{salehi2020lowcomplexity} propose a signal-level coded caching scheme based on predefined placement and delivery matrices, where the file division scales linearly with the number of users. Finally, a general signal-level CC framework is proposed in~\cite{MLPDA_ISIT2022 } based on multi-antenna placement and delivery arrays (MLPDA). As shown in~\cite{MLPDA_ISIT2022 }, any signal-level CC scheme  (including~\cite{lampiris2018adding,salehi2020lowcomplexity,Shahred_cache_Emanuele_2020,Shared_cache_decentrlized_2021}) can be represented with a proper MLPDA.

\noindent\textbf{The near-far issue.}
Another crucial problem of the conventional CC schemes (including~\cite{Shariatpanahi2016,pooya-cc-physical-2019-journal,yu2017exact,tolli2017multi,Ji2016,D2D-CC-Optload-memtradeof-caire-2019,D2D_CC_mahmoodi_2022, PDA_first_2017,cheng_generalized_PDA_2019,DPDA2019,cheng_centralized_PDA_framework_2021,lampiris2018adding,salehi2020lowcomplexity,Shahred_cache_Emanuele_2020,Shared_cache_decentrlized_2021,MLPDA_ISIT2022}) is the \textit{near-far} issue, which affects content delivery applications in general and XR applications in particular. In a nutshell, since in these schemes, a common message is transmitted to serve several users at a time, all these users must be able to decode the message. As a result, the achievable rate is always limited by the user(s) with the worst channel condition. For instance, studies on \ac{SISO}-\ac{CC} networks have shown that the practical gains of CC schemes could entirely vanish at the low--\ac{SNR} region due to the near-far issue~\cite{zhao_petros_MU_MISO_near_far_issue_ITW2021}.  
Thus, aiming to avoid serving users in adverse channel conditions, a congestion control technique is proposed in~\cite{destounis2020adaptive}, partly tackling the near-far issue. Similar scheduling models are also proposed in~\cite{Coded_caching_for_stochastic_wireless_network_TWC2021} and~\cite{liu_joint_power_energi_cc_TWC2021}, where joint queue minimization and packet control, as well as power minimization and scheduling, are introduced for delay-constrained CC applications. Unlike~\cite{destounis2020adaptive,Coded_caching_for_stochastic_wireless_network_TWC2021,liu_joint_power_energi_cc_TWC2021}, in which users with bad wireless connectivity are ignored for data delivery, in~\cite{salehi2020coded}, these users are served with a lower quality of experience (QoE) than the well-conditioned ones.

\noindent\textbf{Multi-rate transmission in \ac{CC}.}
%Using a different perspective, it was discussed in~\cite{ozfatura_mobility_awaire_RCOM2020} that as long as user mobility patterns were known at the server, different cache profiles could be assigned to multiple cache-enabled helper nodes scattered throughout the environment to improve the \ac{CC} transmission rate. Moreover, guiding users towards locations with preferable conditions in an immersive XR application using learning-based techniques was considered in~\cite{reinforcement_for_immersive_elsevier2017}, and an order-optimal location-based coded cache placement was proposed in~\cite{caire_optimal_location_dependent_arxiv2021} to assign different cache profiles to cache-enabled transmitters located in distinct locations. 
In~\cite{Shariatpanahi2016,pooya-cc-physical-2019-journal,yu2017exact,tolli2017multi,Ji2016,D2D-CC-Optload-memtradeof-caire-2019, D2D_CC_mahmoodi_2022, cheng_generalized_PDA_2019, DPDA2019, cheng_centralized_PDA_framework_2021, PDA_first_2017, MLPDA_ISIT2022, lampiris2018adding,salehi2020lowcomplexity,Shahred_cache_Emanuele_2020,Shared_cache_decentrlized_2021}, equal-sized data chunks are combined to form a common message, making the symmetric rate necessary to minimize the overall transmission time and limiting the performance to the users with the worst channel condition. In contrast, in~\cite{tang2017coded}, data with different sizes were combined via nested code modulation (NCM), creating codewords that serve every user in the multicasting group at a different rate. Similarly, combining the shared-cache idea of~\cite{lampiris2018adding} with the NCM of~\cite{tang2017coded}, the near-far problem was mitigated in~\cite{zhao_wireless_CC_ring_area_ISIT2021} and~\cite{zhao_petros_near_far_Nakagami_asilomar2021}. The proposed system model in~\cite{tang2017coded} assumes fixed link capacities, particularly tailored for backhaul networks. Motivated by the results in~\cite{tang2017coded}, authors in~\cite{Mahmoodi_immersive_isit2021} proposed a location-dependent CC network with variable link capacity, particularly applicable for future wireless XR applications. Later, the SISO setting in~\cite{Mahmoodi_immersive_isit2021} was extended to a location-dependent MISO setup in~\cite{mahmoodi_ICC2022_nonsym,mahmoodi2022asymmetric,mahmoodi2022asymmetric_arxiv_TWC2023}. Specifically, while the scheme in~\cite{mahmoodi2022asymmetric} and\cite{mahmoodi2022asymmetric_arxiv_TWC2023} benefits from the NCM for data delivery, the scheme in~\cite{mahmoodi_ICC2022_nonsym} uses a modified version of the signal-level scheme in~\cite{salehi2020lowcomplexity} to support multi-rate transmission. Nevertheless, the scheme proposed in~\cite{mahmoodi2022asymmetric} and\cite{mahmoodi2022asymmetric_arxiv_TWC2023} does not scale with the number of users due to the complex receiver structure. Similarly, the scheme proposed in~\cite{mahmoodi_ICC2022_nonsym} is limited to scenarios where the global caching gain is not greater than the multiplexing gain. Hence, a general framework that can scale with the number of users without a practical limitation still needs to be improved in the literature.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Our contribution}
\label{section:our_contribution}

A novel location-dependent multi-antenna CC scheme is proposed in this paper, leveraging location-aware placement and delivery arrays (LAPDA). The LAPDAs in this work are formed using a proper MLPDA (c.f.,~\cite{PDA_first_2017}), which removes our previous work constraint in~\cite{mahmoodi_ICC2022_nonsym}, i.e., the need for a larger multiplexing gain than global caching gain. We follow the XR connectivity framework proposed in our earlier work~\cite{mahmoodi2022asymmetric_arxiv_TWC2023}. However, unlike~\cite{mahmoodi2022asymmetric_arxiv_TWC2023}, the proposed delivery scheme in this paper utilizes a linear transceiver design with a fast iterative beamforming process, making it suitable for large networks. The proposed scheme is particularly suitable for collaborative XR applications with a moderate/large number of users, where a group of users is served simultaneously in a bounded environment. Specifically, in the considered XR setup,  the actions and choices of each user affect the final results perceived by all the other users. We assume all the users are equipped with cache memories and occasionally move in the application environment. When users change their position in the environment, their wireless connectivity condition changes based on their new location and surrounding obstacles. 

Furthermore, we assume that the environment comprises several single transmission units (STU), where a distinct 3D image is needed in each STU to reconstruct the $360$-degree spherical virtual viewpoint around the user. The required XR content is assumed to be comprised of \textit{static} and \textit{dynamic} parts, where each user needs to acquire both parts to have a detailed field of view (FoV) (c.f., Figure~\ref{fig:static_dynamic_decomposition}). Typically, users can cache both the dynamic and the static parts and render the final result~\cite{flashback_2016_VR_static_dynamic_support}. This paper utilizes multi-antenna \ac{CC} techniques for efficient cache placement and delivery of the \emph{cacheable} content. Similar to any other CC-based scheme, this paper's content delivery comprises two consecutive phases, i.e., \emph{cache placement} and \emph{delivery}. During the delivery phase, users are scattered in the environment, and based on their current locations, they ask the server for the missing data needed to reconstruct their FoVs. Accordingly, the server transmits a downlink (DL) message comprising missing parts for the dynamic and static data and the required instructions for FoV rendering using the cached content. After receiving the DL message, all the users can render their FoVs using cache content and the delivered data. Note that the achievable rate for data delivery varies for different locations. As a result, a novel cache placement and delivery scheme to minimize the average transmission time and avoid excessive delivery duration is proposed in this paper. Hence, the proposed XR framework considers a non-uniform wireless connectivity scenario with location-dependent content requests.

\begin{figure}[t]
     \centering
      \includegraphics[width=1\columnwidth,keepaspectratio]{figs/new dynamic static.pdf}
        \caption{XR Data decomposition into static and dynamic parts.}
        \label{fig:static_dynamic_decomposition}
\end{figure}

Allocating larger cache portions to the contents requested in wireless connectivity bottleneck areas can prevent excessive transmission time. To this end, following the proposed memory allocation process in~\cite{mahmoodi2022asymmetric_arxiv_TWC2023}, a relative rate difference among the different locations of the application environment is first approximated. Then, the content requested in STUs with reduced connectivity is prioritized for cache placement using the approximated rate differences. Then, by defining a set of LAPDAs, novel cache placement and content delivery algorithms are introduced for the resulting non-uniform cache allocation setup. The proposed scheme can achieve a global caching gain additive to the spatial multiplexing gain.

The proposed set of LAPDAs in this paper serves the users via unicast transmissions, resulting in decreased complexity of transceivers. Moreover, a low-complexity iterative beamforming process is proposed based on a weighted max-min optimization. As a result, similar to~\cite{mahmoodi2022asymmetric_arxiv_TWC2023}, users in poor-connectivity STUs are served with smaller amounts of data while simultaneously delivering larger amounts to other users. The proposed delivery scheme in this paper is well suited for large networks due to a simpler transceiver design than~\cite{mahmoodi2022asymmetric_arxiv_TWC2023}. Hence, it is better tailored to the considered XR application scenario with many users. Finally, the proposed delivery method outperforms the conventional symmetric CC schemes despite a \ac{DoF} loss. This is due to avoiding excessive delivery delays to users in areas with poor communication quality.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Notation and structure}
Matrices and vectors are presented by boldface upper and lower case letters, respectively, and calligraphic letters are used to denote sets. For the set $\CA$ and vector $\Bv$, $|\CA|$ and $\|\Bv\|$ represent the cardinality of $\CA$ and norm of $\Bv$, respectively. Also, for two sets $\CA$ and $\CB$, $\CA \backslash \CB$ includes the elements of $\CA$ that are not in $\CB$. Finally, $[m]$ denotes the set of integer numbers $\{1, . . . ,m\}$, and $\oplus$ represents addition in the corresponding finite field. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The rest of this paper is organized as follows.
In section~\ref{sec:sysmodel}, we describe our location-based system model. A two-phase cache placement scheme comprised of memory allocation and cache arrangement processes is described in section~\ref{sec:cache_placement}, while section~\ref{sec:delivery} discusses the delivery procedure. In section~\ref{Sec:beamforming}, weighted-max-min beamforming, tailored for the considered location-based cache placement setup, is introduced. In the end, numerical results are provided in section~\ref{sec:Simulations}, while section~\ref{sec:conclusions} concludes the paper.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

